Learning How to Self-Learn: Enhancing Self-Training Using Neural Reinforcement Learning

Self-training is a useful strategy for semi-supervised learning, leveraging raw texts for enhancing model performances. Traditional self-training methods depend on heuristics such as model confidence for instance selection, the manual adjustment of which can be expensive. To address these challenges, we propose a deep reinforcement learning method to learn the self-training strategy automatically. Based on neural network representation of sentences, our model automatically learns an optimal policy for instance selection. Experimental results show that our approach outperforms the baseline solutions in terms of better tagging performances and stability.

==> Makefile <==
MASTER=naaclhlt2018

TEXS= \
    $(MASTER).tex
    
BIBS = \
    reference.bib 

    
default: $(MASTER).ps

$(MASTER).dvi: $(TEXS) $(EPS_FILES) $(BIBS)
	latex $(MASTER).tex
	bibtex $(MASTER)
	latex $(MASTER).tex
	latex $(MASTER).tex

%.pdf : %.ps
	#./ps2pdf-embedfonts $< $@
	ps2pdf14 -dPDFSETTINGS=/prepress $< $@

%.ps : %.dvi
	dvips -t letter -f < $< > $@

ps: $(MASTER).ps

pdf: $(MASTER).pdf

# Build pdf using pdflatex only (not latex)
pdflatex:
	pdflatex --shell-escape $(MASTER).tex
	bibtex $(MASTER)
	pdflatex --shell-escape $(MASTER).tex
	pdflatex --shell-escape $(MASTER).tex

epsimages := $(wildcard *.eps)
pdfimages := $(epsimages:.eps=.pdf)
clean:
	rm -f *.dvi *.aux $(MASTER).ps $(MASTER).out *.bbl *.blg *.log $(pdfimages)

spell:
	ispell -b -t $(TEXS)

.PHONY: ps pdf pdflatex clean spell



==> cut.tex <==
\begin{tabular}{|c|c|c|c|}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5\hline
     & {\bf English} &  {\bf Dutch} & {\bf Spanish} \\
\hline 
NO SL&  42.54  &  44.56  & 46.83 \\
\hline
RD   &  42.23  &  31.71  & 36.84  \\
\hline
%%%%%%%%%%%%TSL  &  42.57  &  32.48  & 37.35  \\
%%%%%%%%%%%%%%%%%%%%%%%\hline
DQN  &  {\bf 46.28}  &  {\bf 46.06}  & {\bf 46.97}  \\
\hline
\end{tabular}
%%%%%%%%%%%%%%%%%%\caption{Performance comparison for zero-shot NER tagging (\%)}
\label{table:exp1}
\end{table}
\fi

\iffalse

\begin{table}[!t]
\centering

\fi

==> experiment2.tex <==
\section{Experiments}\label{sec:exps}

We conduct two sets of experiments to evaluate our self-training based
proposal for cross lingual %(and POS ?) 
tagging tasks. Note that our self-training approach
is general and can be applied to other sequence labeling tasks. 

\subsection{Data}
For the cross-lingual NER experiments we use the training, 
development and evaluation data sets from the CoNLL 2002/2003 shared tasks 
~\cite{tjong2002data,tjong2003data} for all
four languages: English, German, Spanish and Dutch.  
The data set for each language consists of newswire text annotated with four entity categories: Location (LOC), Miscellaneous (MISC), Organization (ORG) and Person (PER).

%For the cross-domain experiments, we use the SANCL2012 dataset

\subsection{Experimental Settings}
\textbf{Experiment 1.} In the first set of experiments, we use in-domain self-learning approach to train a DQN
for NER tagging in different domains (English, Dutch and Spain,
respectively). Only the dev dataset in each domain has gold
labels and a cross-language pre-trained embedding \cite{Ammar2016MTLDS} is used. To initialize the NER tagger 
in each domain, we randomly select 100 sentences with gold labels from the dev dataset of the domain. Then, we train
the DQN in the domain using the unlabeled data in a self-training way, as depicted in Algorithm~\ref{alg:indomain} . 
%That is,
%when the action of the DQN is to select the input sentence, the NER tagger is
%used to predict the labels for this sentence. This sentence together with the
%predicted labels are then added to the training set to retrain the NER tagger
%and update the parameters of the DQN. 
In each training episode, if the latest 10
rewards in the episode is smaller than a given threshold (0.001), the
performance change is regarded as not significant and this episode is
terminated. To optimize the weights of the DQN, the DQN in each domain is
trained for 10000 episodes. 

Once the DQN for a given domain is trained, we apply it to select sentences from
this domain. The NER tagger is initialized using the
same 100 instances as in the DQN training. 
%Given a stream of unlabeled sentences
%from the training set, if the DQN selects an input sentence, we use the NER
%%agger to predict its labels. This sentence together with its predicted labels
%are then added to the training set to retrain the NER tagger. 
The performance of
the NER tagger is tested and recorded in each step once a sentence is selected
from the unlabeled data set. This procedure is repeated until the number of
selected sentences is larger than a given budget (200).  

To evaluate the effectiveness of the DQN-based solution, we also implement and
test two baseline solutions, i.e., a random solution (denoted as $RD$) and a
confidence-based self-training solution (denoted as $TSL$). In the $TSL$ solution, the confidence is calculated based on the most probable label sequence under the CRF model (NER tagger), i.e. given a unlabeled sentence $x_i$ with $n$ tokens, the confidence is defined as $\sqrt[n]{max_y{p(y|x_i)}}$. In both baseline
approaches, the NER tagger is initialed using the same 100 instances as used in
the DQN-based approach. For the random solution, a stream of input sentences are
randomly selected and tagged by the NER tagger. 
%The selected sentences from the
%unlabeled dataset together with the predicted labels are added to the training
%set to retrain the NER tagger. The procedure is repeated when a given number of
%sentences are randomly selected and added to the training set. 
In the
confidence-based self-training solution, we calculate the confidence of a sentence
using the same approach as in our DQN neural network. Sentences with top
confidences are selected, tagged and added to the training set. To make it
comparable, the number of selected sentences from the unlabeled dataset is the
same in all the three solutions (200). 

\textbf{Experiment 2.} In the second set of experiments, we train the DQN combining the data from the source
and target domains. Similar to Experiment 1, cross-lingual embeddings \cite{Ammar2016MTLDS} are used in the experiment.  
We initialize the NER tagger using the
training set from the source domain (English with gold labels). 
%Then, we train
%the DQNs for three target domains (German, dutch, and Spain) in a self-training
%way using the unlabeled dataset from each domain. Similar to the setting in the
%first experiment, when the DQN selects an unlabeled sentence in the
%target domain, we use the NER tagger trained from the source domain to predict
%its labels. This sentence together with its labels are added to the training
%set. The NER tagger and the DQN is then retrained using the updated training
%set. 
In each training episode, if the latest 10 rewards in the episode is
smaller than a given threshold (0.001), the performance change is regarded not
significant and this episode is terminated. To optimize the weights of the DQN,
the DQN in each target domain is trained for 10000 episodes. 

Once a DQN for a target domain is trained, we use it to select sentences from
the target domain to train the NER model in self-training. Similarly, we
initialize the NER tagger using the dataset from the source domain, then use the DQN to 
select unlabeled sentences from the target domain. The two baseline approaches are similar to those in the
first experiment. The difference is that the initialized NER tagger is trained
from the source domain. The number of sentences
selected from the target domain is the same for all the three approaches (200).
%The selected sentences with the labels
%predicted by the NER tagger are added to the training set to retrain the NER tagger.
%The performance of the NER tagger in each step is tested and recorded. This
%procedure is repeated unless the number of selected sentences is larger than a given
%budget(200).

\begin{figure*}[!t] 
  \centering

    \subfigure[English NER Tagging]{
      \includegraphics[width=0.45\linewidth]{eng405.JPG}
      \label{fig:eng4.05}
   }
%   \subfigure[German NER Tagging]{ 
%      \includegraphics[width=0.45\linewidth]{deu4-05.JPG}
%      \label{fig:deu4.05}
%   }
%\vspace{1mm}
\hspace{3mm}
   \subfigure[Spain NER Tagging]{
      \includegraphics[width=0.45\linewidth]{esp405.JPG}
      \label{fig:esp4.05}
   }
%   \subfigure[Dutch NER Tagging]{ 
%      \includegraphics[width=0.45\linewidth]{ned4-05.JPG}
%      \label{fig:ned4.05}
%   }   
\caption{Self-training for single domain tagging}
\label{fig:exp1}
\end{figure*}


\begin{table}[!t]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
     & English &  Dutch & Spain \\
\hline 
NO SL&  42.54  &  44.56  & 46.83 \\
\hline
RD   &  42.23  &  31.71  & 36.84  \\
\hline
TSL  &  42.57  &  32.48  & 37.35  \\
\hline
DQN  &  46.28  &  46.06  & 46.97  \\
\hline
\end{tabular}
\caption{Performance comparison for in-domain tagging (\%)}
\label{table:exp1}
\end{table}

 
%in the second experiment, we may also add a pos tagging task for gweb-answer dataset.

\subsection{Results}
The results of Experiment 1 are shown in Fig.~\ref{fig:exp1}. In all the
three domains (English, Dutch, and Spain), our DQN-based solution gives a
better performance than the two baseline solutions, as shown in Table~\ref{table:exp1}. Generally, the performance of our solution increases more quickly and drops more slowly than that of the two baseline solutions. In particular, Fig.~\ref{fig:eng4.05} shows that in the English domain, our DQN-based solution has a highest peak performance after
adding 20 unlabeled instances. The unlabeled instances contributes to an
improvement of $4.4\%$ f1-score for the NER tagger. Therefore, our DQN-based
solution can select more useful unlabeled instances to improve the tagger
performance effectively. In the Spain domain, as shown in Fig.~\ref{fig:esp4.05}, the performance of $TSL$ has a slight increase, but drops quickly after
adding 10 unlabeled instances. In contrast, our DQN-based solution behaves more
stably, and the performance increases slowly. 
\iffalse
This may be due to the reason
that the tagging performance of the initial NER model is
not accurate enough to provide useful labels for the sentences selected by both the two baseline solutions. In contrast, our
DQN-based solution selects more useful instances, and the performance of the
tagger is therefore more stable. We also observe in the experiment a similar phenomena in the Dutch domain. 
\fi
%In the
%Dutch domain, although the performance of all the three solutions drops with the
%increasing number of selected unlabeled sentences, the performance of our
%DQN-based solution drops more slowly that the two baseline solutions. Therefore,
%our DQN-based solution has a better strategy to select unlabeled sentences for
%the self-training in single-domain tagging tasks.

\begin{figure*}[!t] 
    \centering
%    \subfigure[English to German Adaptation]{
%      \includegraphics[width=0.45\linewidth]{deu4-1.JPG}
%      \label{fig:deu4.1}
%   }
   \subfigure[English to Spain Adaptation]{ 
      \includegraphics[width=0.45\linewidth]{esp41.JPG}
      \label{fig:esp4.1}
   }
   %\vspace{1mm}
   \hspace{3mm}
   \subfigure[English to Dutch Adaptation]{
      \includegraphics[width=0.45\linewidth]{ned41.JPG}
      \label{fig:ned4.1} 
   }
%  \subfigure[Ontonotes to Gweb Adaptation]{ 
%      \includegraphics[width=0.45\linewidth]{gweb-answer.jpeg}
%      \label{fig:answer}
%   }   

\caption{Self-training for domain adaptation}
\label{fig:exp2}
\end{figure*}




The results of Experiment 2 are shown in Fig.~\ref{fig:exp2}. We can observe that our DQN-based solution has a
better performance than the two baseline solutions, as shown in Table~\ref{table:exp2}. In particular,  
Fig.~\ref{fig:esp4.1} shows the English to Spain adaptation scenario, where the
f1-score of the our DQN-solution increases about $2\%$ and then keeps stable at
about $43.8\%$. In contrast, the F1-score of the two baselines drop dramatically
after adding more unlabeled sentences. Note that although the $TSL$
approach has a sharp increase of performance at the moment of adding 50
unlabeled sentences, it is not stable compared to our DQN-based solution. In the
English to Dutch adaptation scenario, as shown in Fig.~\ref{fig:ned4.1}, we can
observe that all the three approaches have an improvement of the performance
when adding more and more unlabeled sentences. However, our DQN-based solution
still outperforms the two baseline solutions because the performance of our
solution increases more quickly and has a higher peak value than the two baseline solutions.

%Fig.~\ref{fig:answer} shows the POS tagging adaptation from the Ontonotes to
%GWeb-answers dataset. We can observe that the DQN-based solution also
%outperforms the two baseline solutions in the POS tagging scenario.   

We can also observe from Fig.~\ref{fig:exp1} and Fig.~\ref{fig:exp2}
that the DQN-based solution can help to transfer the knowledge from the source
domain to the target domain. For example, as shown in Fig.~\ref{fig:esp4.05} and
Fig.~\ref{fig:esp4.1}, compared to the self-training initialized with 100 annotated sentences from the Spain domain, the NER tagger initialized with the English dataset can
help to achieve a comparable performance without any annotated sentences from the target domain. Table~\ref{table:exp1} and Table~\ref{table:exp2} also show that the NER tagger initialized from the English domain achieves a
lower F1-score than the tagger initialized by 100 sentences from the Dutch
domain. However, self-training using the tagger initialized from the English
domain is more stable. This indicates that the annotated data from the English domain is still helpful to initialize the tagger as a baseline model for a self-training in the target domain. The result also suggests that self-training initialized with a combination of the source training data and a few annotated sentences from the target domain would be worthy further investigation for domain adaptation.

\iffalse
Inspired by this interesting phenomena, we plan to
investigate in the future work how to better combine the dataset from the source
domain and target domain to improve the self-training performance.
\fi
\begin{table}[!t]

\centering
\begin{tabular}{|c|c|c|c|}
\hline
     & Dutch   & Spain   & German \\ 
\hline
NO SL&  33.09  & 41.54   & 31.49 \\
\hline
RD   &  39.42  &  40.36  & 31.51  \\
\hline
TSL  &  38.68  &  41.10  & 31.14 \\ 
\hline
DQN  &  39.86  &  43.33  & 31.58 \\ 
\hline
\end{tabular}
\caption{Performance comparison for cross-domain tagging (\%)}
\label{table:exp2}
\end{table}

==> experiment3.tex <==
\section{Experiments}\label{sec:exps}

We conduct two sets of experiments to evaluate our self-training based
proposal for cross lingual %(and POS ?) tagging tasks. Note that our self-training approach
is general and can be applied to other sequence labeling tasks. 

\subsection{Data}
For the cross-lingual NER experiments we use the training, 
development and evaluation data sets from the CoNLL 2002/2003 shared tasks 
~\cite{tjong2002data,tjong2003data} for all
four languages: English, German, Spanish and Dutch.  
The data set for each language consists of newswire text annotated with four entity categories: Location (LOC), Miscellaneous (MISC), Organization (ORG) and Person (PER).

%For the cross-domain experiments, we use the SANCL2012 dataset

\subsection{In-Domain Tagging}
\textbf{Settings.} In the first set of experiments, we use in-domain self-learning approach to train a DQN
for NER tagging in different domains (English, Dutch and Spanish,
respectively). Only the dev dataset in each domain has gold
labels and a cross-language pre-trained embedding \cite{Ammar2016MTLDS} is used. To initialize the NER tagger 
in each domain, we randomly selected 100 sentences with gold labels from the dev dataset of the domain. Then, we trained the DQN in the domain using the unlabeled data in a self-training way, as depicted in Algorithm~\ref{alg:indomain} . 
%That is,
%when the action of the DQN is to select the input sentence, the NER tagger is
%used to predict the labels for this sentence. This sentence together with the
%predicted labels are then added to the training set to retrain the NER tagger
%and update the parameters of the DQN. 
In each training episode, if the latest 10 rewards in the episode is smaller than a given threshold (0.001), the
performance change is regarded as not significant and this episode is
terminated. To optimize the weights of the DQN, the DQN in each domain is
trained for 10000 episodes. 

Once the DQN for a given domain is trained, we apply it to select sentences from
this domain. The NER tagger is initialized using the
same 100 instances as in the DQN training. 
%Given a stream of unlabeled sentences
%from the training set, if the DQN selects an input sentence, we use the NER
%%agger to predict its labels. This sentence together with its predicted labels
%are then added to the training set to retrain the NER tagger. 
The performance of
the NER tagger is tested and recorded in each step once a sentence is selected
from the unlabeled data set. This procedure is repeated until the number of
selected sentences is larger than a given budget (200).  

To evaluate the effectiveness of the DQN-based solution, we also implement and test two baseline solutions, i.e., a random solution (denoted as $RD$) and a confidence-based self-training solution (denoted as $TSL$). In the $TSL$ solution, the confidence is calculated based on the most probable label sequence under the CRF model (NER tagger), i.e. given a unlabeled sentence $x_i$ with $n$ tokens, the confidence is defined as $\sqrt[n]{max_y{p(y|x_i)}}$. In both baseline
approaches, the NER tagger is initialed using the same 100 instances as used in
the DQN-based approach. For the random solution, a stream of input sentences are
randomly selected and tagged by the NER tagger. 
%The selected sentences from the
%unlabeled dataset together with the predicted labels are added to the training
%set to retrain the NER tagger. The procedure is repeated when a given number of
%sentences are randomly selected and added to the training set. 
In the
confidence-based self-training solution, we calculated the confidence of a sentence
using the same approach as in our DQN neural network. Sentences with top
confidences are selected, tagged and added to the training set. To make it
comparable, the number of selected sentences from the unlabeled dataset is the
same in all the three solutions (200). 

\begin{table}[!t]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
     & {\bf English} &  {\bf Dutch} & {\bf Spanish} \\
\hline 
NO SL&  42.54  &  44.56  & 46.83 \\
\hline
RD   &  42.23  &  31.71  & 36.84  \\
\hline
TSL  &  42.57  &  32.48  & 37.35  \\
\hline
DQN  &  {\bf 46.28}  &  {\bf 46.06}  & {\bf 46.97}  \\
\hline
\end{tabular}
\caption{Performance comparison for in-domain tagging (\%)}
\label{table:exp1}
\end{table}

{\bf Results.} The results of are shown in Table~\ref{table:exp1}. In all the
three domains (English, Dutch, and Spanish), our DQN-based solution gives a
better performance than the two baseline solutions. Generally, the performance of our solution increases more quickly and drops more slowly than that of the two baseline solutions. 

We choose two typical cases and show their learning curves in Fig.~\ref{fig:exp1}. 
In particular, Fig.~\ref{fig:eng4.05} shows that in the English domain, our DQN-based solution has a highest peak performance after
adding 20 unlabeled instances. The unlabeled instances contributes to an
improvement of $4.4\%$ F1-score for the NER tagger. Therefore, our DQN-based
solution can select more useful unlabeled instances to improve the tagger
performance effectively. 

Fig.~\ref{fig:esp4.05} shows a case where self-training did not turn out highly useful, regardless of the strategy. In particular, in the Spanish domain, as shown in Fig.~\ref{fig:esp4.05}, the performance of $TSL$ has a slight increase, but drops quickly after
adding 10 unlabeled instances. In contrast, our DQN-based solution behaves more
stably, and the performance increases slowly. 
\subsection{Cross-Domain Tagging}
\textbf{Settings.} In the second set of experiments, we train the DQN combining the data from the source
and target domains. Similar to Experiment 1, cross-lingual embeddings \cite{Ammar2016MTLDS} are used in the experiment.  
We initialize the NER tagger using the
training set from the source domain (English with gold labels). 
%Then, we train
%the DQNs for three target domains (German, dutch, and Spanish) in a self-training
%way using the unlabeled dataset from each domain. Similar to the setting in the
%first experiment, when the DQN selects an unlabeled sentence in the
%target domain, we use the NER tagger trained from the source domain to predict
%its labels. This sentence together with its labels are added to the training
%set. The NER tagger and the DQN is then retrained using the updated training
%set. 
In each training episode, if the latest 10 rewards in the episode is
smaller than a given threshold (0.001), the performance change is regarded not
significant and this episode is terminated. To optimize the weights of the DQN,
the DQN in each target domain is trained for 10000 episodes. 

Once a DQN for a target domain is trained, we use it to select sentences from
the target domain to train the NER model in self-training. Similarly, we
initialize the NER tagger using the dataset from the source domain, then use the DQN to 
select unlabeled sentences from the target domain. The two baseline approaches are similar to those in the
first experiment. The difference is that the initialized NER tagger is trained
from the source domain. The number of sentences
selected from the target domain is the same for all the three approaches (200).
%The selected sentences with the labels
%predicted by the NER tagger are added to the training set to retrain the NER tagger.
%The performance of the NER tagger in each step is tested and recorded. This
%procedure is repeated unless the number of selected sentences is larger than a given
%budget(200).

\begin{figure*}[!t] 
  \centering

    \subfigure[English NER Tagging]{
      \includegraphics[width=0.45\linewidth]{eng405.JPG}
      \label{fig:eng4.05}
   }
%   \subfigure[German NER Tagging]{ 
%      \includegraphics[width=0.45\linewidth]{deu4-05.JPG}
%      \label{fig:deu4.05}
%   }
%\vspace{1mm}
\hspace{3mm}
   \subfigure[Spanish NER Tagging]{
      \includegraphics[width=0.45\linewidth]{esp405.JPG}
      \label{fig:esp4.05}
   }
%   \subfigure[Dutch NER Tagging]{ 
%      \includegraphics[width=0.45\linewidth]{ned4-05.JPG}
%      \label{fig:ned4.05}
%   }   
\caption{Self-training for single domain tagging}
\label{fig:exp1}
\end{figure*}




 
%in the second experiment, we may also add a pos tagging task for gweb-answer dataset.

\iffalse
This may be due to the reason
that the tagging performance of the initial NER model is
not accurate enough to provide useful labels for the sentences selected by both the two baseline solutions. In contrast, our
DQN-based solution selects more useful instances, and the performance of the
tagger is therefore more stable. We also observe in the experiment a similar phenomena in the Dutch domain. 
\fi
%In the
%Dutch domain, although the performance of all the three solutions drops with the
%increasing number of selected unlabeled sentences, the performance of our
%DQN-based solution drops more slowly that the two baseline solutions. Therefore,
%our DQN-based solution has a better strategy to select unlabeled sentences for
%the self-training in single-domain tagging tasks.
\begin{figure*}[!t] 
    \centering
%    \subfigure[English to German Adaptation]{
%      \includegraphics[width=0.45\linewidth]{deu4-1.JPG}
%      \label{fig:deu4.1}
%   }
   \subfigure[English to Spanish Adaptation]{ 
      \includegraphics[width=0.45\linewidth]{esp41.JPG}
      \label{fig:esp4.1}
   }
   %\vspace{1mm}
   \hspace{3mm}
   \subfigure[English to Dutch Adaptation]{
      \includegraphics[width=0.45\linewidth]{ned41.JPG}
      \label{fig:ned4.1} 
   }
%  \subfigure[Ontonotes to Gweb Adaptation]{ 
%      \includegraphics[width=0.45\linewidth]{gweb-answer.jpeg}
%      \label{fig:answer}
%   }   

\caption{Self-training for domain adaptation}
\label{fig:exp2}
\end{figure*}
\begin{table}[!t]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
     & {\bf Dutch}   & {\bf Spanish}   & {\bf German} \\ 
\hline
NO SL&  33.09  & 41.54   & 31.49 \\
\hline
RD   &  39.42  &  40.36  & 31.51  \\
\hline
TSL  &  38.68  &  41.10  & 31.14 \\ 
\hline
DQN  &  {\bf 39.86}  &  {\bf 43.33}  & {\bf 31.58} \\ 
\hline
\end{tabular}
\caption{Performance comparison for cross-domain tagging (\%)}
\label{table:exp2}
\end{table}
{\bf Results.} The results are shown in Table~\ref{table:exp2}. We can observe that our DQN-based solution has a
better performance than the two baseline solutions. In particular,  
Fig.~\ref{fig:esp4.1} shows the English to Spanish adaptation scenario, where the
F1-score of the our DQN-solution increases about $2\%$ and then keeps stable at
about $43.8\%$. In contrast, the F1-score of the two baselines drop dramatically
after adding more unlabeled sentences. Note that although the $TSL$
approach has a sharp increase of performance at the moment of adding 50
unlabeled sentences, it is not stable compared to our DQN-based solution. In the
English to Dutch adaptation scenario, as shown in Fig.~\ref{fig:ned4.1}, we can
observe that all the three approaches have an improvement of the performance
when adding more and more unlabeled sentences. However, our DQN-based solution
still outperforms the two baseline solutions because the performance of our
solution increases more quickly and has a higher peak value than the two baseline solutions.

%Fig.~\ref{fig:answer} shows the POS tagging adaptation from the Ontonotes to
%GWeb-answers dataset. We can observe that the DQN-based solution also
%outperforms the two baseline solutions in the POS tagging scenario.   

We can also observe from Fig.~\ref{fig:exp1} and Fig.~\ref{fig:exp2}
that the DQN-based solution can help to transfer the knowledge from the source
domain to the target domain. For example, as shown in Fig.~\ref{fig:esp4.05} and
Fig.~\ref{fig:esp4.1}, compared to the self-training initialized with 100 annotated sentences from the Spanish domain, the NER tagger initialized with the English dataset can
help to achieve a comparable performance without any annotated sentences from the target domain. Table~\ref{table:exp1} and Table~\ref{table:exp2} also show that the NER tagger initialized from the English domain achieves a
lower F1-score than the tagger initialized by 100 sentences from the Dutch
domain. However, self-training using the tagger initialized from the English
domain is more stable. This indicates that the annotated data from the English domain is still helpful to initialize the tagger as a baseline model for a self-training in the target domain. The result also suggests that self-training initialized with a combination of the source training data and a few annotated sentences from the target domain would be worthy further investigation for domain adaptation.

\iffalse
Inspired by this interesting phenomena, we plan to
investigate in the future work how to better combine the dataset from the source
domain and target domain to improve the self-training performance.
\fi


==> experiment4.tex <==
\section{Experiments}\label{sec:exps}

We conduct two sets of experiments to evaluate our self-training based
proposal for cross lingual %(and POS ?) tagging tasks. Note that our self-training approach
is general and can be applied to other sequence labeling tasks. 

\subsection{Data}
For the cross-lingual NER experiments we use the training, 
development and evaluation data sets from the CoNLL 2002/2003 shared tasks 
~\cite{tjong2002data,tjong2003data} for all
four languages: English, German, Spanish and Dutch.  
CoNLL 2003 provides English and German sentences.
The data set for each language consists of newswire text annotated with four entity categories: Location (LOC), Miscellaneous (MISC), Organization (ORG) and Person (PER).

%For the cross-domain experiments, we use the SANCL2012 dataset

\subsection{Baselines and Evaluation Metrics}
To evaluate the effectiveness of the DQN-based solution, we also implement and test two baseline solutions, i.e., a random solution (denoted as $RD$) and a confidence-based self-training solution (denoted as $TSL$). In the $TSL$ solution, the confidence is calculated based on the most probable label sequence under the CRF model (NER tagger), i.e. given a unlabeled sentence $x_i$ with $n$ tokens, the confidence is defined as $\sqrt[n]{max_y{p(y|x_i)}}$. 

In both baseline
approaches, the NER tagger is initialed using the same  instances as used in
the DQN-based approach. For the random solution, a stream of input sentences are
randomly selected and tagged by the NER tagger. 
\subsection{In-Domain Tagging}
\textbf{Settings.} We use in-domain self-learning approach to train a DQN
for NER tagging in different domains (English, Dutch and Spanish,
respectively). Only the dev dataset in each domain has gold
labels and a cross-language pre-trained embedding \cite{Ammar2016MTLDS} is used. 

To initialize the NER tagger 
in each domain, we randomly selected 100 sentences with gold labels from the dev dataset of the domain. Then, we trained the DQN in the domain using the unlabeled data in a self-training way, as depicted in Algorithm~\ref{alg:indomain} . 
%That is,
%when the action of the DQN is to select the input sentence, the NER tagger is
%used to predict the labels for this sentence. This sentence together with the
%predicted labels are then added to the training set to retrain the NER tagger
%and update the parameters of the DQN. 
In each training episode, if the latest 10 rewards in the episode is smaller than a given threshold (0.001), the
performance change is regarded as not significant and this episode is
terminated. To optimize the weights of the DQN, the DQN in each domain is
trained for 10000 episodes. 

Once the DQN for a given domain is trained, we apply it to select sentences from
this domain. The NER tagger is initialized using the
same 100 instances as in the DQN training. 
%Given a stream of unlabeled sentences
%from the training set, if the DQN selects an input sentence, we use the NER
%%agger to predict its labels. This sentence together with its predicted labels
%are then added to the training set to retrain the NER tagger. 
The performance of
the NER tagger is tested and recorded in each step once a sentence is selected
from the unlabeled data set. This procedure is repeated until the number of
selected sentences is larger than a given budget (200).  
%The selected sentences from the
%unlabeled dataset together with the predicted labels are added to the training
%set to retrain the NER tagger. The procedure is repeated when a given number of
%sentences are randomly selected and added to the training set. 
In the
confidence-based self-training solution, we calculated the confidence of a sentence
using the same approach as in our DQN neural network. Sentences with top
confidences are selected, tagged and added to the training set. To make it
comparable, the number of selected sentences from the unlabeled dataset is the
same in all the three solutions (200). 

\begin{table}[!t]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
     & {\bf English} &  {\bf Dutch} & {\bf Spanish} \\
\hline 
NO SL&  42.54  &  44.56  & 46.83 \\
\hline
RD   &  42.23  &  31.71  & 36.84  \\
\hline
TSL  &  42.57  &  32.48  & 37.35  \\
\hline
DQN  &  {\bf 46.28}  &  {\bf 46.06}  & {\bf 46.97}  \\
\hline
\end{tabular}
\caption{Performance comparison for in-domain tagging (\%)}
\label{table:exp1}
\end{table}

{\bf Results.} The results are shown in Table~\ref{table:exp1}. In all the
three domains (English, Dutch, and Spanish), our DQN-based solution gives a
better performance than the two baseline solutions. Generally, the performance of our solution increases more quickly and drops more slowly than that of the two baseline solutions. 

We choose two typical cases and show their learning curves in Fig.~\ref{fig:exp1}. 
In particular, Fig.~\ref{fig:eng4.05} shows that in the English domain, our DQN-based solution has a highest peak performance after
adding 20 unlabeled instances. The unlabeled instances contributes to an
improvement of $4.4\%$ F1-score for the NER tagger. Therefore, our DQN-based
solution can select more useful unlabeled instances to improve the tagger
performance effectively. 

Fig.~\ref{fig:esp4.05} shows a case where self-training did not turn out highly useful, regardless of the strategy. In particular, in the Spanish domain, as shown in Fig.~\ref{fig:esp4.05}, the performance of $TSL$ has a slight increase, but drops quickly after
adding 10 unlabeled instances. In contrast, our DQN-based solution behaves more
stably, and the performance increases slowly. 
Though the effects of both $RD$ and $TSL$ are negative, DQN gives slightly  improved accuracies compared with the baselines without using self-training. 
\subsection{Cross-Domain Tagging}
\textbf{Settings.} We train the DQN combining the data from the source
and target domains. Similar to in-domain tagging, cross-lingual embeddings \cite{Ammar2016MTLDS} are used in the experiment.  
We initialize the NER tagger using the
training set from the source domain (English with gold labels). 
%Then, we train
%the DQNs for three target domains (German, dutch, and Spanish) in a self-training
%way using the unlabeled dataset from each domain. Similar to the setting in the
%first experiment, when the DQN selects an unlabeled sentence in the
%target domain, we use the NER tagger trained from the source domain to predict
%its labels. This sentence together with its labels are added to the training
%set. The NER tagger and the DQN is then retrained using the updated training
%set. 
In each training episode, if the latest 10 rewards in the episode is
smaller than a given threshold (0.001), the performance change is regarded not
significant and this episode is terminated. To optimize the weights of the DQN,
the DQN in each target domain is trained for 10000 episodes. 

Once a DQN for a target domain is trained, we use it to select sentences from
the target domain to train the NER model in self-training. Similarly, we
initialize the NER tagger using the dataset from the source domain, then use the DQN to 
select unlabeled sentences from the target domain. The two baseline approaches are similar to those in the
first experiment. The difference is that the initialized NER tagger is trained
from the source domain. The number of sentences
selected from the target domain is the same for all the three approaches (200).
%The selected sentences with the labels
%predicted by the NER tagger are added to the training set to retrain the NER tagger.
%The performance of the NER tagger in each step is tested and recorded. This
%procedure is repeated unless the number of selected sentences is larger than a given
%budget(200).

\begin{figure*}[!t] 
  \centering

    \subfigure[English NER Tagging]{
      \includegraphics[width=0.45\linewidth]{eng4-05.png}
      \label{fig:eng4.05}
   }
%   \subfigure[German NER Tagging]{ 
%      \includegraphics[width=0.45\linewidth]{deu4-05.JPG}
%      \label{fig:deu4.05}
%   }
%\vspace{1mm}
\hspace{3mm}
   \subfigure[Spanish NER Tagging]{
      \includegraphics[width=0.45\linewidth]{esp4-05.png}
      \label{fig:esp4.05}
   }
%   \subfigure[Dutch NER Tagging]{ 
%      \includegraphics[width=0.45\linewidth]{ned4-05.JPG}
%      \label{fig:ned4.05}
%   }   
\caption{Self-training for single domain tagging}
\label{fig:exp1}
\end{figure*}




 
%in the second experiment, we may also add a pos tagging task for gweb-answer dataset.

\iffalse
This may be due to the reason
that the tagging performance of the initial NER model is
not accurate enough to provide useful labels for the sentences selected by both the two baseline solutions. In contrast, our
DQN-based solution selects more useful instances, and the performance of the
tagger is therefore more stable. We also observe in the experiment a similar phenomena in the Dutch domain. 
\fi
%In the
%Dutch domain, although the performance of all the three solutions drops with the
%increasing number of selected unlabeled sentences, the performance of our
%DQN-based solution drops more slowly that the two baseline solutions. Therefore,
%our DQN-based solution has a better strategy to select unlabeled sentences for
%the self-training in single-domain tagging tasks.
\begin{figure*}[!t] 
    \centering
%    \subfigure[English to German Adaptation]{
%      \includegraphics[width=0.45\linewidth]{deu4-1.JPG}
%      \label{fig:deu4.1}
%   }
   \subfigure[English to Spanish Adaptation]{ 
      \includegraphics[width=0.45\linewidth]{esp4-1.png}
      \label{fig:esp4.1}
   }
   %\vspace{1mm}
   \hspace{3mm}
   \subfigure[English to Dutch Adaptation]{
      \includegraphics[width=0.45\linewidth]{ned4-1.png}
      \label{fig:ned4.1} 
   }
%  \subfigure[Ontonotes to Gweb Adaptation]{ 
%      \includegraphics[width=0.45\linewidth]{gweb-answer.jpeg}
%      \label{fig:answer}
%   }   

\caption{Self-training for domain adaptation}
\label{fig:exp2}
\end{figure*}
\begin{table}[!t]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
     & {\bf Dutch}   & {\bf Spanish}   & {\bf German} \\ 
\hline
NO SL&  33.09  & 41.54   & 31.49 \\
\hline
RD   &  39.42  &  40.36  & 31.51  \\
\hline
TSL  &  38.68  &  41.10  & 31.14 \\ 
\hline
DQN  &  {\bf 39.86}  &  {\bf 43.33}  & {\bf 31.58} \\ 
\hline
\end{tabular}
\caption{Performance comparison for cross-domain tagging (\%)}
\label{table:exp2}
\end{table}
{\bf Results.} The results are shown in Table~\ref{table:exp2}. We can observe that our DQN-based solution has a
better performance than the two baseline solutions. In particular,  
Fig.~\ref{fig:esp4.1} shows the English to Spanish adaptation scenario, where the
F1-score of the our DQN-solution increases about $2\%$ and then keeps stable at
about $43.8\%$. In contrast, the F1-score of the two baselines drop dramatically
after adding more unlabeled sentences. Note that although the $TSL$
approach has a sharp increase of performance at the moment of adding 50
unlabeled sentences, it is not stable compared to our DQN-based solution. In the
English to Dutch adaptation scenario, as shown in Fig.~\ref{fig:ned4.1}, we can
observe that all the three approaches have an improvement of the performance
when adding more and more unlabeled sentences. However, our DQN-based solution
still outperforms the two baseline solutions because the performance of our
solution increases more quickly and has a higher peak value than the two baseline solutions.

%Fig.~\ref{fig:answer} shows the POS tagging adaptation from the Ontonotes to
%GWeb-answers dataset. We can observe that the DQN-based solution also
%outperforms the two baseline solutions in the POS tagging scenario.   

We can also observe from Fig.~\ref{fig:exp1} and Fig.~\ref{fig:exp2}
that the DQN-based solution can help to transfer the knowledge from the source
domain to the target domain. For example, as shown in Fig.~\ref{fig:esp4.05} and
Fig.~\ref{fig:esp4.1}, compared to the self-training initialized with 100 annotated sentences from the Spanish domain, the NER tagger initialized with the English dataset can
help to achieve comparable performances without any annotated sentences from the target domain. Table~\ref{table:exp1} and Table~\ref{table:exp2} also show that the NER tagger initialized from the English domain achieves a
lower F1-score than the tagger initialized by 100 sentences from the Dutch
domain. However, self-training using the tagger initialized from the English
domain is more stable. This indicates that the annotated data from the English domain is still helpful to initialize the tagger as a baseline model for a self-training in the target domain. The result also suggests that self-training initialized with a combination of the source training data and a few annotated sentences from the target domain would be worthy further investigation for domain adaptation.

\iffalse
Inspired by this interesting phenomena, we plan to
investigate in the future work how to better combine the dataset from the source
domain and target domain to improve the self-training performance.
\fi


==> experiment5.tex <==
\section{Experiments}\label{sec:exps}

%We conduct two sets of experiments to evaluate our self-training based
%proposal for in-domain and cross-domain tagging. 


\subsection{Data}
For the cross-lingual NER experiments we use the training, 
development and evaluation data sets from the CoNLL 2002/2003 shared tasks 
~\cite{tjong2002data,tjong2003data} for all
four languages: English, German, Spanish and Dutch.  
The data set for each language consists of newswire text annotated with four entity categories: Location (LOC), Miscellaneous (MISC), Organization (ORG) and Person (PER).

%For the cross-domain experiments, we use the SANCL2012 dataset

\subsection{Baselines, Hyperparameters and Evaluation Metrics}
To evaluate the effectiveness of the DQN-based solution, we also implement and test two baseline solutions, i.e., a random solution (denoted as $RD$) and a confidence-based self-training solution (denoted as $TSL$).  

In both baseline approaches, the NER tagger is initialed using the same instances as used in
the DQN-based approach. For the $RD$ solution, a stream of input sentences are
randomly selected and tagged by the NER tagger. 
In the $TSL$ solution, the confidence is calculated based on the most probable label sequence under the Bi-lstm CRF model (NER tagger), the same as in our DQN neural network. That is. given a unlabeled sentence $x_i$ with $n$ tokens, the confidence is defined as $\sqrt[n]{max_y{p(y|x_i)}}$. Sentences with top
confidences are selected, tagged and added to the training set. 

During each training episode of a DQN, if the latest 10 rewards in the episode is smaller than a given threshold (0.001), the performance change is regarded as not significant and this episode is terminated. To optimize the weights of a DQN, the DQN is trained for 10000 episodes. 

Once a DQN for a specific task is trained, we apply it to select automatically labeled sentences. The NER tagger is initialized using the same instances as used in the DQN training. 
The performance of the NER tagger is tested and recorded in each step once a sentence is selected from the unlabeled data set. To make it comparable, the number of selected sentences from the unlabeled dataset is the same in all the three solutions (200).

\subsection{In-Domain Tagging}
\textbf{Settings.} We use in-domain self-learning approach to train a DQN
for NER tagging in different domains (English, Dutch and Spanish,
respectively). Only the dev dataset in each domain has gold
labels and a cross-language pre-trained embedding \cite{Ammar2016MTLDS} is used. 
In each domain, we randomly selected 100 sentences with gold labels from the dev dataset of the domain as the initial annotation data. Then, we trained the DQN in the domain using the unlabeled data in a self-training way, as depicted in Algorithm~\ref{alg:indomain} . 
%That is,
%when the action of the DQN is to select the input sentence, the NER tagger is
%used to predict the labels for this sentence. This sentence together with the
%predicted labels are then added to the training set to retrain the NER tagger
%and update the parameters of the DQN. 
%In each training episode, if the latest 10 rewards in the episode is smaller than a given threshold (0.001), the
%performance change is regarded as not significant and this episode is
%terminated. To optimize the weights of the DQN, the DQN in each domain is
%trained for 10000 episodes. 

%Once the DQN for a given domain is trained, we apply it to select sentences from
%this domain. The NER tagger is initialized using the
%same 100 instances as in the DQN training. 
%Given a stream of unlabeled sentences
%from the training set, if the DQN selects an input sentence, we use the NER
%%agger to predict its labels. This sentence together with its predicted labels
%are then added to the training set to retrain the NER tagger. 
%The performance of
%the NER tagger is tested and recorded in each step once a sentence is selected
%from the unlabeled data set. This procedure is repeated until the number of
%selected sentences is larger than a given budget (200).  
%The selected sentences from the
%unlabeled dataset together with the predicted labels are added to the training
%set to retrain the NER tagger. The procedure is repeated when a given number of
%sentences are randomly selected and added to the training set. 
 
\begin{table}[!t]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
     & {\bf English} &  {\bf Dutch} & {\bf Spanish} \\
\hline 
NO SL&  42.54  &  44.56  & 46.83 \\
\hline
RD   &  42.23  &  31.71  & 36.84  \\
\hline
TSL  &  42.57  &  32.48  & 37.35  \\
\hline
DQN  &  {\bf 46.28}  &  {\bf 46.06}  & {\bf 46.97}  \\
\hline
\end{tabular}
\caption{Performance comparison for in-domain tagging (\%)}
\label{table:exp1}
\end{table}

{\bf Results.} The results are shown in Table~\ref{table:exp1}. In all the
three domains (English, Dutch, and Spanish), our DQN-based solution gives a
better performance than the two baseline solutions. Generally, the performance of our solution increases more quickly and drops more slowly than that of the two baseline solutions. 

We choose two typical cases and show their learning curves in Fig.~\ref{fig:exp1}. 
In particular, Fig.~\ref{fig:eng4.05} shows that in the English domain, our DQN-based solution has a highest peak performance after
adding 20 unlabeled instances. The unlabeled instances contributes to an
improvement of $4.4\%$ F1-score for the NER tagger. Therefore, our DQN-based
solution can select more useful unlabeled instances to improve the tagger
performance effectively. 

Fig.~\ref{fig:esp4.05} shows a case where self-training did not turn out highly useful, regardless of the strategy. In particular, in the Spanish domain, as shown in Fig.~\ref{fig:esp4.05}, the performance of $TSL$ has a slight increase, but drops quickly after
adding 10 unlabeled instances. In contrast, our DQN-based solution behaves more
stably, and the performance increases slowly. 
Though the effects of both $RD$ and $TSL$ are negative, DQN gives slightly improved accuracies compared with the baselines without using self-training. 
\subsection{Cross-Domain Tagging}
\textbf{Settings.} We train the DQN combining the data from the source
and target domains. Similar to in-domain tagging, cross-lingual embeddings \cite{Ammar2016MTLDS} are used in the experiment.  
We initialize the NER tagger using the
training set from the source domain (English with gold labels). 
%Then, we train
%the DQNs for three target domains (German, dutch, and Spanish) in a self-training
%way using the unlabeled dataset from each domain. Similar to the setting in the
%first experiment, when the DQN selects an unlabeled sentence in the
%target domain, we use the NER tagger trained from the source domain to predict
%its labels. This sentence together with its labels are added to the training
%set. The NER tagger and the DQN is then retrained using the updated training
%set. 
%In each training episode, if the latest 10 rewards in the episode is
%smaller than a given threshold (0.001), the performance change is regarded not
%significant and this episode is terminated. To optimize the weights of the DQN,
%the DQN in each target domain is trained for 10000 episodes. 

%Once a DQN for a target domain is trained, we use it to select sentences from
%the target domain to train the NER model in self-training. Similarly, we
%initialize the NER tagger using the dataset from the source domain, then use the DQN to 
%select unlabeled sentences from the target domain. The two baseline approaches are similar to those in the
%first experiment. The difference is that the initialized NER tagger is trained
%from the source domain. The number of sentences
%selected from the target domain is the same for all the three approaches (200).
%The selected sentences with the labels
%predicted by the NER tagger are added to the training set to retrain the NER tagger.
%The performance of the NER tagger in each step is tested and recorded. This
%procedure is repeated unless the number of selected sentences is larger than a given
%budget(200).

\begin{figure*}[!t] 
  \centering

    \subfigure[English NER Tagging]{
      \includegraphics[width=0.45\linewidth]{eng4-05.png}
      \label{fig:eng4.05}
   }
%   \subfigure[German NER Tagging]{ 
%      \includegraphics[width=0.45\linewidth]{deu4-05.JPG}
%      \label{fig:deu4.05}
%   }
%\vspace{1mm}
\hspace{3mm}
   \subfigure[Spanish NER Tagging]{
      \includegraphics[width=0.45\linewidth]{esp4-05.png}
      \label{fig:esp4.05}
   }
%   \subfigure[Dutch NER Tagging]{ 
%      \includegraphics[width=0.45\linewidth]{ned4-05.JPG}
%      \label{fig:ned4.05}
%   }   
\caption{Self-training for single domain tagging}
\label{fig:exp1}
\end{figure*}




 
%in the second experiment, we may also add a pos tagging task for gweb-answer dataset.

\iffalse
This may be due to the reason
that the tagging performance of the initial NER model is
not accurate enough to provide useful labels for the sentences selected by both the two baseline solutions. In contrast, our
DQN-based solution selects more useful instances, and the performance of the
tagger is therefore more stable. We also observe in the experiment a similar phenomena in the Dutch domain. 
\fi
%In the
%Dutch domain, although the performance of all the three solutions drops with the
%increasing number of selected unlabeled sentences, the performance of our
%DQN-based solution drops more slowly that the two baseline solutions. Therefore,
%our DQN-based solution has a better strategy to select unlabeled sentences for
%the self-training in single-domain tagging tasks.
\begin{figure*}[!t] 
    \centering
%    \subfigure[English to German Adaptation]{
%      \includegraphics[width=0.45\linewidth]{deu4-1.JPG}
%      \label{fig:deu4.1}
%   }
   \subfigure[English to Spanish Adaptation]{ 
      \includegraphics[width=0.45\linewidth]{esp4-1.png}
      \label{fig:esp4.1}
   }
   %\vspace{1mm}
   \hspace{3mm}
   \subfigure[English to Dutch Adaptation]{
      \includegraphics[width=0.45\linewidth]{ned4-1.png}
      \label{fig:ned4.1} 
   }
%  \subfigure[Ontonotes to Gweb Adaptation]{ 
%      \includegraphics[width=0.45\linewidth]{gweb-answer.jpeg}
%      \label{fig:answer}
%   }   

\caption{Self-training for domain adaptation}
\label{fig:exp2}
\end{figure*}
\begin{table}[!t]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
     & {\bf Dutch}   & {\bf Spanish}   & {\bf German} \\ 
\hline
NO SL&  33.09  & 41.54   & 31.49 \\
\hline
RD   &  39.42  &  40.36  & 31.51  \\
\hline
TSL  &  38.68  &  41.10  & 31.14 \\ 
\hline
DQN  &  {\bf 39.86}  &  {\bf 43.33}  & {\bf 31.58} \\ 
\hline
\end{tabular}
\caption{Performance comparison for cross-domain tagging (\%)}
\label{table:exp2}
\end{table}
{\bf Results.} The results are shown in Table~\ref{table:exp2}. We can observe that our DQN-based solution has a
better performance than the two baseline solutions. In particular,  
Fig.~\ref{fig:esp4.1} shows the English to Spanish adaptation scenario, where the
F1-score of the our DQN-solution increases about $2\%$ and then keeps stable at
about $43.8\%$. In contrast, the F1-score of the two baselines drop dramatically
after adding more unlabeled sentences. Note that although the $TSL$
approach has a sharp increase of performance at the moment of adding 50
unlabeled sentences, it is not stable compared to our DQN-based solution. In the
English to Dutch adaptation scenario, as shown in Fig.~\ref{fig:ned4.1}, we can
observe that all the three approaches have an improvement of the performance
when adding more and more unlabeled sentences. However, our DQN-based solution
still outperforms the two baseline solutions because the performance of our
solution increases more quickly and has a higher peak value than the two baseline solutions.

%Fig.~\ref{fig:answer} shows the POS tagging adaptation from the Ontonotes to
%GWeb-answers dataset. We can observe that the DQN-based solution also
%outperforms the two baseline solutions in the POS tagging scenario.   

We can also observe from Fig.~\ref{fig:exp1} and Fig.~\ref{fig:exp2}
that the DQN-based solution can help to transfer knowledge from the source
domain to the target domain. For example, as shown in Fig.~\ref{fig:esp4.05} and
Fig.~\ref{fig:esp4.1}, compared to the self-training initialized with 100 annotated sentences from the Spanish domain, the NER tagger initialized with the English dataset can
help to achieve comparable performances without any annotated sentences from the target domain. Table~\ref{table:exp1} and Table~\ref{table:exp2} also show that the NER tagger initialized from the English domain achieves a
lower F1-score than the tagger initialized by 100 sentences from the Dutch
domain. However, self-training using the tagger initialized from the English
domain is more stable. This indicates that the annotated data from the English domain is still helpful to initialize the tagger as a baseline model for a self-training in the target domain. 
\iffalse
The result also suggests that self-training initialized with a combination of the source training data and a few annotated sentences from the target domain would be worthy further investigation for domain adaptation.


Inspired by this interesting phenomena, we plan to
investigate in the future work how to better combine the dataset from the source
domain and target domain to improve the self-training performance.
\fi


==> introduction.tex <==

\section{Introduction}\label{section:intro}     
    
There is a need for semi-supervised learning when a target domain or language    
lacks of manual resources. 
Self-training is a commonly used strategy. 
It can improve results of a model trained using a set of existing labeled data, by    
adding to the training data a set of raw data automatically labeled by the    
baseline model.    
    
In traditional self-training approaches, the baseline model is initialized based    
on a few instances with gold labels. The baseline model is used to tag all the    
unlabeled data from the unlabeled training set. The automatically labeled    
instances are then selected based on some strategies and added to retrain the    
baseline model. The self-training procedure is repeated until the number of    
selected automatically labeled instances reaches a budget. Self-training has    
different strategies for selecting automatically labeled data, such as the    
confidence value of the baseline model. Theoretically, it resembles EM giving    
local minimum.    
    
The crucial point of a self-training approach is how to define and measure the    
confidence of an automatically labelling, since this may be due to many factors    
varying from tasks to tasks. Therefore, existing self-training solutions are    
usually designed manually based on the heuristics in particular task settings.    
This leads to two draw backs of self-training: 1.  Manual adjustment of instance    
selection strategy is costly. 2. For the best effect on a unknown dataset the    
source of information is limited to model confidence and a few other simple    
heuristics. As a result, the design of an effective self-training strategy    
manually is challenging.    
    
Since the design of an effective self-training approach is challenging, can we    
learn a self-training approach automatically without human heuristics? Note that    
a self-training approach can be regarded as a decision process, which decides in    
each step what automatically labeled instances can be selected. This decision    
process can be represented as a function that receives the automatically labeled    
instances as input and outputs the indexes of the selected instances. Based on    
this observation, we therefore consider learning this function automatically    
instead of designing it manually. In this paper, we present our efforts    
to learn the function for a self-training approach automatically. Since no human    
heuristics are needed in the training, and the training dataset has no gold    
labels, feedback is needed to help make an effective decision. Therefore,    
we investigate using deep reinforcement learning to automatically select    
instances for a given task. The basis is the performance improvements on a set    
of development data after a certain set of automatically labeled data are added    
to the training instances.    
    
Compared with manual heuristics, a deep model is capable of automatically    
learning the characteristics of training instances, and hence can potentially be    
more flexible in choose the most useful data. Therefore, our approach is more    
general and can be applied to different NLP tasks. To evaluate the effectiveness    
of our proposal, we design two self-training algorithms for two typical NLP    
tasks: self-training for in-domain tagging and self-learning for cross-domain    
adaptation. We apply our solution to NER tagging and POS tagging in these    
scenarios. The experimental results show that our approach outperforms the    
baseline solutions in terms of a better tagging performance and being more stable.    

The remainder of this paper is organized as follow:    
Section~\ref{sec:RW} reviews the state-of-the-art literature on
self-training and reinforcement learning for NLP tasks. Section~\ref{sec:method}
introduces our self-training methodology, elaborating in detail how the deep
reinforcement learning neural network for self-training is designed.
Section~\ref{sec:exps} presents our experimental setup and result analysis.
Section~\ref{sec:conclusion} concludes the work and highlights some potential
research issues.


==> introduction0.tex <==


\section{Introduction}\label{section:intro}

- There is a need for semi-supervised learning when a target domain or language lacks manual resources. Self-Training is a commonly used strategy. It can lead to improved results of a model trained using a set of existing labeled data, by adding to the training data a set of raw data automatically labeled by the baseline model.

- Self training has different strategies for selecting automatically labeled data, such as the confidence value of the baseline model. Theoretically, it resembles EM giving local minimum…

Two draw backs of self-training. 1. Manual adjustment of instance selection strategy is costly. 2. For the best effect on a unknown dataset the source of information is limited to model confidence and a few other simple heuristics. 

We investigate using deep reinforcement learning to automatically select instances for a given task. The basis is the performance improvements on a set of development data after a certain set of automatically labeled data are added to the training instances. 

Compared with manual heuristics, a deep model is capable of automatically learning the characteristics of training instances, and hence can potentially be more flexible in choose the most useful data. 



In many NLP application tasks, it is difficult to obtain sufficient annotated
texts. Therefore, many semi-supervisied and unsupervised learning approaches 
are developed to extract useful information from unlabeled dataset. Among these
approaches, self-learning is regarded as a promising approach to train the model
based on the unlabeled data.

%In traditional self-learning approaches, a model is initialized based on a few
%instances with gold labels. This initialized model is then used to tag all the
%unlabeled data from the training set. The unlabeled instances with top
%confidence for the tagging are added to the training set, together with the
%labels tagged by the initialized tagger. The updated training dataset is then
%used to retrain the tagger. The procedure is repeated until the training reaches
%a budget. 
The crucial point of a self-learning approach is how to define and
measure the confidence of a tagging, since this may be due to many factors and
these factors may vary from tasks to tasks. Therefore, existing self-learning
solutions are usually designed manually based on the heuristics in particular
task settings. This introduces a challenge to apply these approaches to a
different setting. As a result, new human heuristics and efforts are needed from
different applications.

Since the design of an efficient self-learning approach is challenging, can we
learn a self-learning approach automatically without human heuristics? Note that
a self-learning approach can be regarded as a decision process, where in each
step the approach selects some instances, tag them and add them to the training
set. This decision process can be represented as a function that receives the
unlabeled instances as input and outputs the indexes of the selected instances.
Based on this observation, we therefore consider learning this function
automatically instead of designing it by human efforts. In this paper, we
present our efforts to learn the function for a self learning approach
automatically. Since no human heuristics are needed in the training, and the
training dataset has no gold labels, feedbacks are needed to help decide whether
the selection of an unlabeled instance contributes to the performance
improvement. Therefore, we train the self-learning decision function based on
reinforcement learning framework. We propose a deep reinforcement learning
neural network to capture the heuristics hidden in the unlabeled data and
training procedure automatically.

Our approach is general and can be applied to different NLP tasks. To evaluate
the effectiveness of the proposal, we design two self-learning algorithms for
two typical application scenarios: self learning for in-domain tagging and
self-learning for cross-domain adaptation. We apply our solution to named entity recognition 
and part-of-speech tagging in these scenarios. The experimental results show that our
approach outperforms the baseline solutions.

The remainder of this paper is organized as follow:
Section~\ref{sec:RW} reviews the state-of-the-art literatures on
self-learning and reinforcement learning for NLP tasks. Section~\ref{sec:method}
introduces our methodology, elaborating in detail how the deep reinforcement
learning neural network for self-learning is designed. Section~\ref{sec:exps}
presents our experimental setup and result analysis.
Section~\ref{sec:conclusion} concludes the work and highlights the potential
research issues. 




%Self-learning leverages well trained taggers to provide pseudo-labels to unlabeled samples.
%Add the instances in which the current algorithm is the most confident, 
%Assign pseudo-labels to unlabeled samples get domain, and train the neural networks as if they are true labels.
%
%
%With deep reinforcement learning, we can likely learn an  query policy for any given data-sets. 
%Thus a classifier that performs well on various domains.
%
%In many scenarios of interest data is hard to obtain, so agents may learn a
%source policy in a setting where data is readily available, 
%with the hope that it generalizes well to the target domain.
%We would like to be able to leverage our trained model in the source domain
%to inform the predictions of a new model trained on the target domain.
%
%Also in some scenario, true labels in the target domain are not available. 
%That is also called unsupervised domain adaptation problem.
%The self-learning via reinforcement learning framework to .... 
%
%
%Much research efforts have been devoted to transfer learning or domain adaptation 
%for NLP task ~\cite{Ardehaly2016DomainAF}.
%
%The appeal of the domain adaptation approaches is 
%the ability to learn a mapping between domains in the situation 
%when the target domain data are either fully unlabeled (unsupervised domain annotation) 
%or have few labeled samples (semi-supervised domain adaptation). 
%
%
%We show that this method is robust across 5 domains for part of speech tagging and 4 languages for named
%entity recognition.


==> introduction1.tex <==

\section{Introduction}\label{section:intro}     
    
Semi-supervised learning is useful for improving model performances when a target domain or language lacks of manual resources. 
Self-training is a commonly used strategy for various natural language processing tasks, such as named entity recognition (NER) \cite{kozareva2005self}, part-of-speech (POS) tagging \cite{wang2007semi,qi2009semi} and parsing \cite{McClosky2006parsing,mcclosky2008self,Huang2009latentpcfg,Sagae2010parseradaptation}.

%It can potentially improve the baseline models which train using a set of existing labeled data, by    
%augmenting the training data with a set of raw data automatically labeled by the baseline model.    
The basic idea of self-training is to augment the original training set with
a set of automatic predictions of high confidence.  
In particular, traditional self-training approaches train the baseline models using a few instances with gold labels. 
Then the baseline models are used to predict a set of unlabeled data.  
The automatically labeled instances are filtered based on some strategies and added to the training set for retraining new baseline models. 
This procedure continues until the number of automatically labeled instances reaches a budget or the model performance becomes stable.  Theoretically, it resembles EM, giving local minimum.    

Self-training has different strategies for selecting automatically labeled data, such as the confidence values of the baseline models. 
How to define and measure the confidence of predictions is the crucial point of a successful self-training approach. 
The selection methods depends on many factors, varying from tasks to tasks.
Therefore, traditional self-training solutions are usually designed manually based on the task-specific heuristics \cite{rosenberg2005semi,Ardehaly2016domainadaptation,Jason2011emnlp,medlock2007weakly,daume2008cross}.     
This leads to two draw backs of self-training: 1) manual adjustment of instance selection strategy is costly; 2) for the best effect on a unknown dataset, the  source of information is limited to model confidence and a few other simple heuristics. 
As a result, the manual design of an effective self-training strategy remains  challenging.    
    
%In this paper,  we learn a self-training approach automatically without human heuristics. 
Note that a self-training approach can be regarded as a decision process, where each step decides which automatically labeled instances can be selected. 
This decision process can be represented as a function that receives the automatically labeled instances as inputs and outputs a signal to indicate the acceptance or rejection of the prediction result.  
Based on this observation, we therefore consider learning this function automatically    
instead of designing it manually. 
In this paper, we present our efforts to learn the function for a self-training approach automatically. 
Since no human heuristics are needed in the training, and the training dataset  has no gold  labels, feedback is needed to help make an effective decision. 
Therefore, we investigate deep Q-network \cite{nature14,guo2015generating,fang2017activelearning} to automatically select instances for a given task. 
The basis is the performance improvements on a set    
of development data after a certain set of automatically labeled data are added    
to the training instances.    
    
Compared with manual heuristics, the deep Q-network model is capable of automatically learning the characteristics of training instances, and hence can potentially be more flexible in choose the most useful data. 
Therefore, our approach is more general and can be applied to different NLP tasks. 
To evaluate the effectiveness of our proposal, we design two self-training algorithms for two typical NLP tasks: self-training for in-domain tagging and self-training for cross-domain adaptation. 
We apply our solution to NER tagging and POS tagging in these  scenarios. 
The experimental results show that our approach outperforms the baseline solutions in terms of a better tagging performance and being more stable.    

The remainder of this paper is organized as follow:    
Section~\ref{sec:RW} reviews the state-of-the-art literature on
self-training and reinforcement learning for NLP tasks. Section~\ref{sec:method}
introduces our self-training methodology, elaborating in detail how the deep
 Q-network for self-training is designed. 
Section~\ref{sec:exps} presents our experimental setup and result analysis. 
Section~\ref{sec:conclusion} concludes the work and highlights some potential
research issues. 

==> introduction2.tex <==

\section{Introduction}\label{section:intro}     
    
Scarcity of annotated data has motivated research into techniques capable
of exploiting unlabeled data, e.g., domain adaptation, semi-supervised and
unsupervised learning. Semi-supervised learning is useful for improving model performances when a target domain or language lacks of manual resources. 
Self-training is a commonly used strategy for various natural language processing (NLP) tasks, such as named entity recognition (NER) \cite{kozareva2005self}, part-of-speech (POS) tagging \cite{wang2007semi,qi2009semi} and parsing \cite{McClosky2006parsing,mcclosky2008self,Huang2009latentpcfg,Sagae2010parseradaptation}.

%It can potentially improve the baseline models which train using a set of existing labeled data, by    
%augmenting the training data with a set of raw data automatically labeled by the baseline model.    
The basic idea of self-training is to augment the original training set with
a set of automatic predictions of high confidence.  
In particular, traditional self-training approaches train baseline models using a few instances with gold labels. 
Then the baseline models are used to predict a set of unlabeled data.  
The automatically labeled instances are filtered based on certain strategies and then added to the training set for retraining new baseline models. 
This procedure continues until the number of automatically labeled instances reaches a budget or the model performance becomes stable.  Theoretically, it resembles expectation–maximization (EM), giving local minimum to the training objective.    

There has been different strategies for selecting automatically labeled data, such as the confidence values of the baseline models. 
How to define and measure the confidence of predictions is  crucial for a successful self-training approach. 
The selection methods depends on many factors, varying from task to task. 
Therefore, traditional self-training solutions can be designed manually based on task-specific heuristics \cite{rosenberg2005semi,Ardehaly2016domainadaptation,Jason2011emnlp,medlock2007weakly,daume2008cross}.     
This leads to two drawbacks: 1) manual adjustment of instance selection strategy is costly; 2) for the best effect on an  unknown dataset, the  source of information is limited to model confidence and a few other simple heuristics. 
As a result, linguistic characteristics of specific test sentences cannot be captured.    
    
We aim to address this issue by leveraging neural models to represent test sentences, using reinforcement learning to automatically learn instance selection strategy. In particular, a self-training approach can be regarded as a decision process, where each step decides which automatically labeled instances can be selected. 
This decision process can be represented as a function that receives the automatically labeled instances as inputs and outputs a signal to indicate the acceptance or rejection of the prediction result.  
Since no gold  labels exist for instance selection, we use  deep Q-network \cite{nature14,guo2015generating,fang2017activelearning} to learn selection strategy automatically, on the basis of the performance improvements on a set    
of development data.    
    

To evaluate the effectiveness of our proposal, we design two self-training algorithms for two typical NLP tasks: self-training for in-domain tagging and self-training for cross-domain adaptation. 
We apply our solution to NER tagging in these  scenarios. 
The results show that our approach outperforms the baseline solutions in terms of a better tagging performance and stability.  
Compared with manual heuristics, the deep Q-network model is capable of automatically learning the characteristics of training instances, and hence can potentially be more flexible in choose the most useful data. 
Therefore, our approach is more general and can be applied to different NLP tasks. We release our code at http://anonymized. 

The remainder of this paper is organized as follow:    
Section~\ref{sec:RW} reviews the state-of-the-art literature on
self-training and reinforcement learning for NLP tasks. Section~\ref{sec:slmethod} provides some background on the self-training process. Section~\ref{sec:dqnmethod}
introduces our self-training methodology, elaborating in detail how the deep
 Q-network for self-training is designed. 
Section~\ref{sec:exps} presents our experimental setup and result analysis. 
Section~\ref{sec:conclusion} concludes the work and highlights some potential
research issues. 

==> introduction3.tex <==

\section{Introduction}\label{section:intro}     
    
Scarcity of annotated data has motivated research into techniques capable
of exploiting unlabeled data, e.g., domain adaptation, semi-supervised and
unsupervised learning. Semi-supervised learning is useful for improving model performances when a target domain or language lacks of manual resources. 
Self-training is a commonly used strategy for various natural language processing (NLP) tasks, such as named entity recognition (NER) \cite{kozareva2005self}, part-of-speech (POS) tagging \cite{wang2007semi,qi2009semi} and parsing \cite{McClosky2006parsing,mcclosky2008self,Huang2009latentpcfg,Sagae2010parseradaptation}.

%It can potentially improve the baseline models which train using a set of existing labeled data, by    
%augmenting the training data with a set of raw data automatically labeled by the baseline model.    
The basic idea of self-training is to augment the original training set with
a set of automatic predictions of high confidence.  
In particular, traditional self-training approaches train baseline models using a few instances with gold labels. 
Then the baseline models are used to predict a set of unlabeled data.  
The automatically labeled instances are filtered based on certain strategies and then added to the training set for retraining new baseline models. 
This procedure continues until the number of automatically labeled instances reaches a budget or the model performance becomes stable.  Theoretically, it resembles expectation\text{-}maximization (EM), giving local minimum to the training objective.    

There have been different strategies for selecting automatically labeled data, such as the confidence values of the baseline models. 
How to define and measure the confidence of predictions is  crucial for a successful self-training approach. 
The selection methods depends on many factors, varying from task to task. 
Therefore, traditional self-training solutions can be designed manually based on task-specific heuristics \cite{rosenberg2005semi,Ardehaly2016domainadaptation,Jason2011emnlp,medlock2007weakly,daume2008cross}.     
This can lead to two drawbacks: 1) manual adjustment of instance selection strategy is costly; 2) the  source of information is limited to model confidence and a few other simple heuristics. 
As a result, linguistic characteristics of specific test sentences cannot be captured.    
    
We aim to address this issue by leveraging neural models (i.e. convolutional neural network) to represent individual test sentences, using reinforcement learning to automatically learn instance selection strategy. In particular, a self-training approach can be regarded as a decision process, where each step decides which automatically labeled instances can be selected. 
This decision process can be represented as a function that receives the automatically labeled instances as inputs and outputs a signal to indicate the acceptance or rejection of the prediction result.  
Since no gold  labels exist for instance selection, we use  deep Q-network \cite{nature14,guo2015generating,fang2017activelearning} to learn selection strategy automatically, on the basis of the performance improvements on a set    of development data.    
    

To evaluate the effectiveness of our proposal, we design two self-training algorithms for two typical NLP tasks: self-training for in-domain tagging and self-training for cross-domain adaptation. 
We apply our solution to NER tagging in these  scenarios. 
The results show that our approach outperforms the baseline solutions in terms of a better tagging performance and stability.  
Compared with manual heuristics, the deep Q-network model is capable of automatically learning the characteristics of training instances, and hence can potentially be more flexible in choosing the most useful data. 
Therefore, our approach is more general and can be applied to different NLP tasks. We release our code at http://anonymized. 

The remainder of this paper is organized as follow:    
Section~\ref{sec:RW} reviews the state-of-the-art literature on
self-training and reinforcement learning for NLP tasks. Section~\ref{sec:slmethod} provides some background on the self-training process. Section~\ref{sec:dqnmethod}
introduces our self-training methodology, elaborating in detail how the deep
 Q-network for self-training is designed. 
Section~\ref{sec:exps} presents our experimental setup and result analysis. 
Section~\ref{sec:conclusion} concludes the work and highlights some potential
research issues. 

==> method.tex <==
\section{Self-Training}\label{sec:method}
%This section elaborates our deep reinforcement learning approach for self-training.

%\subsection{Self-Training}
%formalize the problem as a self-learning problem
As explained in Section~\ref{section:intro}, we investigate how to learn a
self-training approach that can be applied to multiple scenarios where the gold
labels are not available and the efforts for human to annotate the labels are
expensive. Our goal is to retrieve useful information from the massive  unlabeled
dataset to improve the training performance.

In traditional self-training framework (Algorithm~\ref{alg:tsl}), a tagger is first initialized using a set of instances with gold labels. Then, this tagger is used to tag a set of unlabeled data, and the confidence of the tagging for each unlabeled instance is evaluated. The automatically labeled instance with highest confidence is added to the
training set, together with the labels predicted by the tagger. Correspondingly, the unlabeled instance is removed from the unlabeled dataset. 
The tagger is
retrained using the updated training dataset and used to tag and select the
unlabeled instances from the remaining dataset. This procedure is repeated until
a given number of instances are selected and added to the training dataset. 

How to measure the confidence of a tagging is crucial to a self-training
approach. Traditional self-training approach usually needs human efforts to
design specific confidence metrics based on the heuristics and application
scenarios. This however is challenging and the effectiveness of the solution
may depend on many factors, which however is not well investigated yet. In this
paper, we propose to learn a self-training strategy automatically. 

%In traditional self-learning framework, the selection of an unlabeled instance
%can be regarded as a decision process, in the sense that the learning strategy
%decides whether an unlabeled instance is added to the training dataset or not in
%each step. Also, the selection of an unlabeled instance in current step depends
%on the selection of an unlabeled instance in the previous step, since the tagger is
%retrained once an unlabeled instance is selected and added to the training
%dataset. Therefore, a self-learning procedure can be regarded as a function that
%takes the current state of the self-learning framework as input and generates
%the output indicating whether an unlabeled instance is selected or not. In
%traditional self-learning approaches, this function is usually designed manually
%with some heuristics. In this paper, we propose to learn this function
%automatically using a deep reinforcement learning network. 

\begin{algorithm}[!t] 
\caption{Traditional self-training}
\label{alg:tsl}
\KwIn{dataset train $T$, dev $D$, budget; unlabeled data $U$}
randomly shuffle $U$\;
\While{$i < budget$ and $U$ is not empty}{
    $tagger\leftarrow train(T)$\;
    $tag(tagger,U)$ \;
    $x_i \leftarrow select(U)| max_{x_i}confidence(y_i)$\;
    $T \leftarrow T \cup (x_i, y_i)$\;
    $U \leftarrow U \backslash (x_i, y_i)$\;
    $i \leftarrow i + 1$\;
}
\KwOut{A self-training tagger;}
\end{algorithm}

\subsection{Deep Reinforcement Learning Framework}

%In a self-training framework, the selection of an unlabeled instance
%can be regarded as a decision process, in the sense that the learning strategy
%decides whether an unlabeled instance is added to the training dataset or not in
%each step. Therefore, a self-training procedure can be regarded as a function that
%takes the current state of the self-learning framework as input and generates
%the output indicating whether an unlabeled instance is selected or not. In
%traditional self-training approaches, this function is usually designed manually
%with some heuristics. In this section, we propose to learn this function
%automatically using a deep reinforcement learning neural network. 

In order to learn a self-training function automatically, we design a deep
reinforcement learning neural network to optimize the function parameters based on the
feedback from the training. 
To formalize the self-training function easily, we
adopt a stream-based strategy. That is, the unlabeled training dataset is
regarded as a stream of instances. For every arriving unlabeled instance, the
self-training function generates an output indicating whether this instance is
selected or not. Given a stream of unlabeled dataset, our goal is to train the
function that can make the decision automatically with a good performance via
reinforcement learning.

%an introduction to reinforcement learning 
{\bf Training Goal} Reinforcement learning has been well adopted to learn a policy function in many
applications scenarios. In this paper, similar to the setting in
~\cite{fang2017activelearning}, we adopt the deep Q-learning approach~\cite{nature14} as our
learning framework (denoted as DQN). In this learning framework, the policy
function $\pi$ is defined via a Q-function: $Q^{\pi}(s,a)\to R$, where $s$ is
the current state of learning framework, $a$ is the action, and $R$ is the
reward of the framework when taking action $a$ from the current state $s$. The
training of the policy function $\pi$ is to find the parameters that can
maximize the reward of the each action in every state. This is done by
iteratively updating $Q^{\pi}(s,a)$ using the rewards obtained from the
sequence of actions during the training, based on the Bellman equation defined
as follows: 
\begin{equation} 
    Q^{\pi}(s,a) = \mathbb{E}[R_i|s_i=s, a_i=a, \pi]
\end{equation} 
where $R_i = \sum_{t=i}^T \gamma^{t-i} r_t$ is the discounted
future rewards and $\gamma\in[0,1]$ is the discounting rate. 

\subsection{Model Structure}

We follow the setting in the deep Q-learning approach~\cite{nature14} to
calculate the expected $Q$ value to update the parameters. We implement the
Q-function using a three-layered neural network, as shown in Fig.~\ref{fig:dqn}.

\begin{figure*}[!t] 
\centering
\includegraphics[width=0.7\linewidth]{qnet3.png}
\caption{The neural network for Q-function}
\label{fig:dqn}
\end{figure*}

%state
The input layer represents the state of the learning framework. We adopt a
similar approach proposed in~\cite{fang2017activelearning} to define the state of the
framework. That is, the state $s$ consists of three parts ($h_s$, $h_c$, $h_p$),
where $h_s$ is the content representation of the arriving instance, $h_c$ is the
confidence of tagging the instance using the tagger, and $h_p$ is the marginals
of the prediction for this instance.

As shown in Fig.~\ref{fig:dqn}, to represent the content of an arriving
instance, a CNN with 384 filters are designed with the size of (3, 4, 5), 128
for each size respectively. Each filter uses a linear transformation with a
rectified linear unit activation function. The input to the CNN is the
concatenated word embedding of the instance via looking up a pre-trained word
embedding. These filters are used to extract the features of the instance
contents. The filter outputs are then merged using a max-pooling operation to
yield a hidden state $h_s$, a vector of size 384 that represents the
content of this instance.

The confidence of the tagger for an instance $h_c$ is defined based on the most
probable label sequence for this instance. In this paper, we adopt in the
experiment a CRF tagger and its confidence value can be output directly from the
CRF tagger. This value can be also defined and measured for different taggers. 

The marginals of the prediction for an instance is also calculated based on a
CNN. The labels of the arriving instance are predicted using the tagger and 20
filters with a size of 3 are designed to extract the features in the prediction.
These feature maps are then sub-sampled with mean pooling to capture the average
uncertainty in each filter. The final hidden layer $h_p$ is used to represent
the predictive marginals. 

%action
The three parts of the state $s=(h_s, h_c, h_p)$ are then used to calculate the
second layer with a rectified linear unit activation function. This hidden layer
is designed as a vector of size 256. Then it is used to calculate expected
Q-value in the output layer, a vector of size 2, indicating whether the
instance should be selected or not. If an instance is selected, the predicted
labels of the sentences together with this sentence are added to the training
set to retrain the tagger.

{\bf Reward} To train this neural network via reinforcement learning, we need to define the
reward for each action. If an instance is not selected, then the reward is set
to 0; otherwise, the reward of this action is defined as the performance
difference of the tagger after the instance is added to the training set. 

%budget for each episode (significance test) 

Following the approach in ~\cite{nature14}, we train the DQN using an experience
replay mechanism. The current state, its actions and corresponding rewards are
recorded in a memory. The parameters of DQN are learned using stochastic
gradient descent to match the Q-values predicted by the DQN and the expected
Q-values from the Bellman equation, $r_i + \gamma max_aQ(s_{i+1}, a; \theta)$.
Samples are randomly selected from the experience memory to update the
parameters of the DQN by minimizing the loss function:
\begin{equation}
    \mathbb{L}(\theta) = (r+ max_{a'}Q(s',a')-Q(s,a))^2
\end{equation}    
The training procedure is repeated with the incoming instances. We conduct a
significance test to decide whether the training episode should be terminated.
In the significance test, we calculate the performance difference between a
series of consecutive actions. If the performance difference of the tagger is
not significant, we terminate the training episode and restart the training with
a new episode.

%may add an algorithm here
\begin{algorithm}[!t] 
\caption{Self training for in-domain tagging}
\label{alg:indomain}
\KwIn{unlabeled data $U$, dev set $D$, test set $T$;}
\KwOut{A self-training tagger;}
%\Begin{
    randomly select a subset $init$ from $D$\;
    $ds \leftarrow init$\; 
    //training DQN\\
    \While {$episode < 10000$} { 
        $tagger\leftarrow train(ds)$\;
        $performance \leftarrow test(tagger, D)$\;
        \While {$!significant(performance)$}{
             $x \leftarrow U$\; 
             $qvalue \leftarrow DQN(x)$\;
             \If{ $argmax(qvalue) == 1$} {
                 $y \leftarrow tag(tagger, x)$\;
                 $ds \leftarrow ds (x, y)$ \;
                 $tagger \leftarrow train(ds)$\;
                 $reward \leftarrow test(tagger, D) - performance$\;
                 $update(DQN, reward)$\;
             }    
        }

        $episode$ += 1\;
    }   

    //train the final tagger\\
    $ds \leftarrow init$\; 
    $tagger \leftarrow train(ds)$\;
    \While {$has(budget)$} { 
        $x \leftarrow U$\;
        $qvalue \leftarrow DQN(x)$\;
        \If {$argmax(qvalue) == 1$} {
             $y \leftarrow tag(tagger,x)$\;
             $ds \leftarrow ds \cup (x, y)$ \;
             $tagger\leftarrow train(ds)$\;
        }    
    }
%}    
\end{algorithm}


\subsection{Tasks}

The deep reinforcement learning neural network for self-learning (denoted as
DQN) can be used to many application scenarios where the gold labels are not
available and the efforts to annotate the labels are expensive. In this section,
we illustrate two application scenarios.

\textbf{Self Training for In-domain Tagging}
In this scenario, the gold label of the training dataset is not available. Only
a small development and test dataset is annotated with gold labels. In this
scenario, we need to apply a self-learning approach to train a tagger that can
be used to tag the unlabeled instances with an acceptable performance.

Algorithm~\ref{alg:indomain} illustrates our solution. In order to learn the
self-learning approach for this scenario, we randomly select a small number of
instances with gold labels from the development dataset. These instances are
then used to initialize the tagger for the self-training. Whenever an unlabeled instance is selected and added to the training set to retrain the tagger, the
performance difference of the tagger on the development data set is calculated
as reward of the action. The reward is regarded as a feedback of the action and
is used to update the parameters of the DQN neural network. The DQN neural
network is self-trained for a given number of episodes. Once the training of the
DQN is finished, we use it to select unlabeled instances from the training
dataset and train the tagger based on those selected unlabeled instances
(together with their predicted labels).


    


\textbf{Self Training for Cross-domain Adaptation}

In this scenario, we have a source domain with a training set full of gold
labels, but the target domain has only a small development set equipped with
gold labels. In this scenario, we need to apply a self-learning approach to
transfer the knowledge learned from the source domain to the target domain. 

The algorithm is similar to Algorithm~\ref{alg:indomain}, the difference is that
we train the tagger using the training dataset from the source domain. The
purpose is to transfer the knowledge from the source domain to the target
domain. 
%Then, this tagger is set as the initialized tagger to train the DQN
%using the unlabeled data from the target domain. If the DQN selects an unlabeled
%instance, the tagger is used to tag this instance. This instance and the
%predicted labels are then added to the training set to retrain the tagger.
%Similarly, the performance difference is calculated as the feedback of the
%action and used to update the parameters of the DQN neural network. 
The DQN neural network is also self-trained for a given number of episodes. Once the training of the DQN is finished, we use the DQN to select unlabeled instances from the
target domain. These selected instances are added together with the training
dataset from the source domain to train the tagger for the target domain.

%may add an algorithm here


==> method0.tex <==
%\section{Method} 

%In this section, we begin with a semi-supervised approach and describe the self-learning understand reinforcement
%learning framework to automatically annotate target domain datasets. 
%The algorithm maintains and grows a training set that is iteratively adapted to the target domain. 
%
%
%Co-training for Domain Adaptation Each iteration, only inputs that are confident according
%to exactly one of the two classifiers are moved to the training set.  
%This way, one classifier provides the (estimated) labels to the inputs on which the
%other classifier is uncertain.
%The main intuition is to train two classifiers on a single view
%such that: (1) both perform well on the labeled data; (2) both are trained on strictly different
%features; (3) together they are likely to satisfy Balcan’s condition ofexpandability, a necessary
%and sufficient pre-condition for co-training to workThese three aspects can be formulated explicitly as three modifications of our optimization problem.
%
%Further, we introduce pseudo multi-view co-training,
%which improves the rote-learning procedure by adding inputs with features that are still not used
%effectively by the current classifier. We use automated feature decomposition to artificially split our
%data into multiple views, explicitly to enable successful co-training.
%
%There are several ways in which our  “best classifier” can be utilized.  
%Our first approach uses this classifier as the initializer  while doing (online)
%active learning in the target domain.
%Then we present a variant augmenting  the first approach using a domain-separator hypothesis which leads to
%additionally ruling out querying the labels of those target examples that appear “similar” to the source
%domain.
%Figure1 shows our basic setup which uses a source classifier v0 as an initializer for doing active learning
% in the target domain having  some  small labeled data set.  
%Our framework consists of 2  phases:   
%1)  Learning  the  best  possible  classifier v0 using source labeled (LS) and unlabeled data(US), 
%and target unlabeled (UT) data, 
%and 2) Querying labels for target domain examples 
%by leveraging information from the classifier learned in phase.
%
%Self-training, as a single-view semi-supervised learning method, has been widely
%used in NLP research. In self-training, an underlying classifier is first
%trained with  a small number of labeled data which is also called the  initial
%training set. The underlying classifier is used to classify the unlabeled data.
%The most confident unlabeled instances with their predicted labels are added to
%the training set. The underlying classifier is then re-trained and the procedure
%repeats. The following is the general procedure of self-training algorithm.
%
%This section provides some background on the active learning process,
%as well as detailing the various sampling strategies we investigate.



\section{Method}\label{section:method}
This section elaborates our deep reinforcement learning approach for self-learning.

\subsection{Self-Training}
%formalize the problem as a self-learning problem
As explained in ~\ref{section:introduction}, we investigate how to learn a
self-learning approach that can be applied to multiple scenarios where the gold
labels are not available and the efforts for human to annotate the labels are
expensive. Our goal is to retrieve useful information from the  unlabeled
dataset to improve the training performance.

In traditional self-learning framework, a tagger is first initialized using some
instances with gold labels. Then, this tagger is used to tag all the unlabeled
data from the training set and the confidence of the tagging for each unlabeled
instance is evaluated. The unlabeled instance with highest confidence is added to the
training set, together with the labels predicted by the tagger. The tagger is
retrained using the updated training dataset and used to tag and select the
unlabeled instances from the remaining dataset. This procedure is repeated until
a given number of instances are selected and added to the training dataset. 

How to measure the confidence of a tagging is crucial to a self-learning
approach. Traditional self-learning approach usually needs human efforts to
design specific confidence metrics based on the heuristics and application
scenarios. This however is challenging and the effectiveness of the solution
may depend on many factors, which however is not well investigated yet. In this
paper, we propose to learn a self-learning automatically. 

In traditional self-learning framework, the selection of an unlabeled instance
can be regarded as a decision process, in the sense that the learning strategy
decides whether an unlabeled instance is added to the training dataset or not in
each step. Also, the selection of an unlabeled instance in current step depends
on the selection of an unlabeled instance in the previous step, since the tagger is
retrained once an unlabeled instance is selected and added to the training
dataset. Therefore, a self-learning procedure can be regarded as a function that
takes the current state of the self-learning framework as input and generates
the output indicating whether an unlabeled instance is selected or not. In
traditional self-learning approaches, this function is usually designed manually
with some heuristics. In this paper, we propose to learn this function
automatically using a deep reinforcement learning network. 


\subsection{Deep Reinforcement Learning Framework}

In order to learn a self-learning function automatically, we design a deep
reinforcement learning network to optimize the function parameters based on the
feedbacks from the training. To formalize the self-learning function easily, we
adopt a stream-based strategy. That is, the unlabeled training dataset is
regarded as a stream of instances. For every arriving unlabeled instance, the
self-learning function generates an output indicating whether this instance is
selected or not. Given a stream of unlabeled dataset, our goal is to train the
function that can make the decision automatically with a good performance via
reinforcement learning.

%an introduction to reinforcement learning 

Reinforcement learning has been well adopted to learn a policy function in many
applications scenarios. In this paper, similar to the setting in
~\cite{emnlp17}, we adopt the deep Q-learning approach~\cite{nature14} as our
learning framework. In this learning framework, the policy function $\pi$ is
defined via a Q-function: $Q^{\pi}(s,a)\to R$, where $s$ is the current state of
learning framework, $a$ is the action, and $R$ is the reward of the framework
when taking action $a$ from the current state $s$. The training of the policy
function $\pi$ is to find the parameters that can maximize the reward of the
each action in every state. This is done by iteratively updating $Q^{\pi}(s,a)$
using the rewards obtained from the sequence of actions during the training,
based on the Bellman equation defined as follows:
\begin{equation}
   Q^{\pi}(s,a) = \mathbb{E}[R_i|s_i=s, a_i=a, \pi]
\end{equation}
where $R_i = \sum_{t=i}^T \gamma^{t-i} r_t$ is the discounted future rewards and
$\gamma\in[0,1]$ is the discounting rate. 

We follow the setting in the deep Q-learning approach~\cite{nature14} to
calculate the expected $Q$ value to update the parameters. We implement the
Q-function using a three-layered neural network, as shown in Fig.~\ref{fig:dqn}.

\begin{figure}[t] 
\centering
\includegraphics[width=0.9\linewidth]{\figpath/dqn}
\caption{The neural network for Q-function}
\label{fig:dqn}
\end{figure}

%state
The input layer represents the state of the learning framework. We adopt a
similar approach proposed in ~\cite{emnlp17} to define the state of the
framework. That is, the state $s$ consists of three parts ($h_s$, $h_c$, $h_p$),
where $h_s$ is the content representation of the arriving instance, $h_c$ is the
confidence of tagging the instance using the tagger, and $h_p$ is the marginals
of the prediction for this instance.

As shown in Fig.~\ref{fig:dqn}, to represent the content of an arriving
instance, a CNN with 384 filters are designed with the size of (3, 4, 5), 128
for each size respectively. Each filter uses a linear transformation with a
rectified linear unit activation function. The input to the CNN is the
concatenated word embedding of the instance via looking up a pre-trained word
embeddings. These filters are used to extract the features of the instance
contents. The filter outputs are then merged using a max-pooling operation to
yield a hidden state $h_s$, a vector of size 384 that represents the
content of this instance.

The confidence of the tagger for an instance $h_c$ is defined based on the most
probable label sequence for this instance. In this paper, we adopt in the
experiment a CRF tagger and its confidence value can be output directly from the
CRF tagger. This value can be also defined and measured for different taggers. 

The marginals of the prediction for an instance is also calculated based on a
CNN. The labels of the arriving instance are predicted using the tagger and 20
filters with a size of 3 are designed to extract the features in the prediction.
These feature maps are then sub-sampled with mean pooling to capture the average
uncertainty in each filter. The final hidden layer $h_p$ is used to represent
the predictive marginals. 

%action
The three parts of the state $s=(h_s, h_c, h_p)$ are then used to calculate the
second layer with a rectified linear unit activation function. This hidden layer
is designed as a vector of size 256. Then it is used to calculate expected
Q-value in the output layer, a vector of size 2, indicating whether the
instance should be selected or not. If an instance is selected, the predicted
labels of the sentences together with this sentence are added to the training
set to retrain the tagger.

%reward
To train this neural network via reinforcement learning, we need to define the
reward for each action. If an instance is not selected, then the reward is set
to 0; otherwise, the reward of this action is defined as the performance
difference of the tagger after the instance is added to the training set. 

%budget for each episode (significance test)
Following the approach in ~\cite{nature14}, we train this neural network using
an experience replay mechanism. The current state, its actions and corresponding
rewards are recorded in a memory. Samples are randomly selected from this memory
to update the parameters of the neural network. The training procedure is repeated
with the incoming instances. We conduct a significance test to decide whether the
training episode should be terminated. In the significance test, we calculate
the performance difference between a series of consecutive actions. If the
performance difference of the tagger is not significant, we terminate the
training episode and restart the training with a new episode. 


\subsection{Applications}

The deep reinforcement learning neural network for self-learning (denoted as
DQN) can be used to many application scenarios where the gold labels are not
available and the efforts to annotate the labels are expensive. In this section,
we illustrate two application scenarios.

\textbf{Self Learning for In-domain Tagging}
In this scenario, the gold label of the training dataset is not available. Only
a small development and test dataset is annotated with gold labels. In this
scenario, we need to apply a self-learning approach to train a tagger that can
be used to tag the unlabeled instances with an acceptable performance.

In order to learn the self-learning approach for this scenario, we randomly
select a small number of instances with gold labels from the development
dataset. These instances are then used to initialize the tagger. This tagger is
then used to tag the unlabeled instances from the training set. Whenever an
instance is selected and tagged, this instance is added to the training set to
retrain the tagger. The performance difference of the tagger on the development
data set is calculated as reward of the action. The reward is regarded as a
feedback of the action and is used to update the parameters of the DQN neural
network. The DQN neural network is self-learned for a given number of episodes. Once
the training of the DQN is finished, we use it to select unlabeled instances
from the training dataset and train the tagger based on those selected unlabeled
instances (together with their predicted labels).

%may add an algorithm here

\textbf{Self Learning for Cross-domain Adaptation}

In this scenario, we have a source domain with a training set full of gold
labels, but the target domain has only a small development set equipped with
gold labels. In this scenario, we need to apply a self-learning approach to
transfer the knowledge learned from the source domain to the target domain. 

In order to transfer the knowledge from the source domain, we train the tagger
using the training dataset from the source domain. Then, this tagger is set as
the initialized tagger to train the DQN using the unlabeled data from the target
domain. If the DQN selects an unlabeled instance, the tagger is used to tag
this instance. This instance and the predicted labels are then added to the
training set to retrain the tagger. Similarly, the performance difference is
calculated as the feedback of the action and used to update the parameters of
the DQN neural network. The DQN neural network is self-learned for a given
number of episodes. Once the training of the DQN is finished, we use the DQN to
select unlabeled instances from the target domain. These selected instances are
added together with the training dataset from the source domain to train the
tagger for the target domain.

%may add an algorithm here




==> method2.tex <==
\section{Self-training}\label{sec:slmethod}
%formalize the problem as a self-learning problem
As explained in Section~\ref{section:intro}, we investigate how to learn a
self-training approach that can be applied to multiple scenarios where the gold
labels are not available and the efforts for human to annotate the labels are
expensive. Our goal is to retrieve useful information from the massive  unlabeled
dataset to improve the training performance.

In traditional self-training framework (Algorithm~\ref{alg:tsl}), a tagger is first initialized using a set of 
instances with gold labels. Then, this tagger is used to tag a set of unlabeled
data,  and the tagging confidence for each unlabeled
instance is evaluated. The automatically labeled instances  with highest confidence is added to the
training set. 
The tagger is
retrained using the updated training dataset and used to tag and select the
unlabeled instances from the remaining dataset. This procedure is repeated until
a given number of instances are selected and added to the training dataset. 

How to measure the confidence of a tagging is crucial to a self-training
approach. Traditional self-training approach usually requires human efforts to
design specific confidence metrics based on the heuristics and application
scenarios. This, however, is challenging and the effectiveness of the solution
may depend on many factors, which however is not well investigated yet. We propose to learn a self-training strategy automatically. 

%In traditional self-learning framework, the selection of an unlabeled instance
%can be regarded as a decision process, in the sense that the learning strategy
%decides whether an unlabeled instance is added to the training dataset or not in
%each step. Also, the selection of an unlabeled instance in current step depends
%on the selection of an unlabeled instance in the previous step, since the tagger is
%retrained once an unlabeled instance is selected and added to the training
%dataset. Therefore, a self-learning procedure can be regarded as a function that
%takes the current state of the self-learning framework as input and generates
%the output indicating whether an unlabeled instance is selected or not. In
%traditional self-learning approaches, this function is usually designed manually
%with some heuristics. In this paper, we propose to learn this function
%automatically using a deep reinforcement learning network. 

\begin{algorithm}[!t] 
\caption{Traditional self-training}
\label{alg:tsl}
\KwIn{dataset train $T$, dev $D$, budget; unlabeled data $U$}
randomly shuffle $U$\;
\While{$i < budget$ and $U$ is not empty}{
    $tagger\leftarrow train(T, D)$\;
    $tag(tagger,U)$ \;
    $x_i \leftarrow select(U)| \max_{x_i}{\it confidence}(y_i)$\;
    $T \leftarrow T \cup (x_i, y_i)$\;
    $U \leftarrow U \backslash (x_i, y_i)$\;
    $i \leftarrow i + 1$\;
}
\KwOut{A self-training tagger;}
\end{algorithm}

\section{Learning how to self-training}\label{sec:dqnmethod}

%In a self-training framework, the selection of an unlabeled instance
%can be regarded as a decision process, in the sense that the learning strategy
%decides whether an unlabeled instance is added to the training dataset or not in
%each step. Therefore, a self-training procedure can be regarded as a function that
%takes the current state of the self-learning framework as input and generates
%the output indicating whether an unlabeled instance is selected or not. In
%traditional self-training approaches, this function is usually designed manually
%with some heuristics. In this section, we propose to learn this function
%automatically using a deep reinforcement learning neural network. 

In order to learn a self-training function automatically, we design a deep
reinforcement learning neural network to optimize the function parameters based on the
feedback from the training. 
To formalize the self-training function easily, we
adopt a stream-based strategy. That is, the unlabeled training dataset is
regarded as a stream of instances. For every arriving unlabeled instance, the
self-training function generates an output indicating whether this instance is
selected or not. Given a stream of unlabeled dataset, our goal is to train the
function that can make the decision automatically with a good performance via
reinforcement learning.

\begin{figure*}[!t] 
\centering
\includegraphics[width=0.7\linewidth]{qnet3.png}
\caption{The neural network for Q-function}
\label{fig:dqn}
\end{figure*}

%an introduction to reinforcement learning 
{\bf Training Goal} Reinforcement learning has been well adopted to learn a policy function in many
applications scenarios. In this paper, similar to the setting in
~\cite{fang2017activelearning}, we adopt the deep Q-learning approach~\cite{nature14} as our
learning framework (denoted as DQN). In this learning framework, the policy
function $\pi$ is defined via a Q-function: $Q^{\pi}(s,a)\to R$, where $s$ is
the current state of learning framework, $a$ is the action, and $R$ is the
reward of the framework when taking action $a$ from the current state $s$. The
training of the policy function $\pi$ is to find the parameters that can
maximize the reward of the each action in every state. This is done by
iteratively updating $Q^{\pi}(s,a)$ using the rewards obtained from the
sequence of actions during the training, based on the Bellman equation defined
as follows: 
\begin{equation} 
    Q^{\pi}(s,a) = \mathbb{E}[R_i|s_i=s, a_i=a, \pi]
\end{equation} 
where $R_i = \sum_{t=i}^T \gamma^{t-i} r_t$ is the discounted
future rewards and $\gamma\in[0,1]$ is the discounting rate. 



\subsection{Model Structure}

We follow the setting in the deep Q-learning approach~\cite{nature14} to
calculate the expected $Q$ value to update the parameters. We implement the
Q-function using a three-layered neural network, as shown in Fig.~\ref{fig:dqn}.

%state
The input layer represents the state of the learning framework. We adopt a
similar approach proposed by \newcite{fang2017activelearning} to define the state of the
framework. In particular, a state $s$ consists of three elements ($h_s$, $h_c$, $h_p$),
where $h_s$ is the content representation of the arriving instance, $h_c$ is the
confidence of tagging the instance using the tagger, and $h_p$ is the marginals
of the prediction for this instance.

As shown in Fig.~\ref{fig:dqn}, to represent the content of an arriving
instance, a convolutional neural network (CNN) with 384 filters are designed, with the convolution size being (3, 4, 5), and 128 filters 
for each size, respectively. Each filter uses a linear transformation with a
rectified linear unit activation function. The input to the CNN is the
concatenated word embedding of the instance via looking up a pre-trained word
embedding. These filters are used to extract the features of the instance
contents. The filter outputs are then merged using a max-pooling operation to
yield a hidden state $h_s$, a vector of size 384 that represents the
content of this instance.

The confidence of the tagger for an instance $h_c$ is defined based on the most
probable label sequence for this instance. In this paper, we adopt in the
experiment a CRF tagger and its confidence value can be taken directly from the
CRF tagger. This value can be also defined and measured for different taggers. 

The marginals of the prediction for an instance is also calculated based on a
CNN. The labels of the arriving instance are predicted using the tagger and 20
filters with a size of 3 are designed to extract the features in the prediction.
These feature maps are then sub-sampled with mean pooling to capture the average
uncertainty in each filter. The final hidden layer $h_p$ is used to represent
the predictive marginals. 

%action
The three elements of the state $s=(h_s, h_c, h_p)$ are then used to calculate the
second layer with a rectified linear unit activation function. This hidden layer
is designed as a vector of size 256. Then it is used to calculate expected
Q-value in the output layer, a vector of size 2, indicating whether the
instance should be selected or not. If an instance is selected, the predicted
labels of the sentences together with this sentence are added to the training
set to retrain the tagger.

{\bf Reward} To train this neural network via reinforcement learning, we need to define the
reward for each action. If an instance is not selected, then the reward is set
to 0; otherwise, the reward of this action is defined as the performance
difference of the tagger after the instance is added to the training set. 

%budget for each episode (significance test) 

Following the approach of \newcite{nature14}, we train the DQN using an experience
replay mechanism. The current state, its actions and corresponding rewards are
recorded in a memory. The parameters of DQN are learned using stochastic
gradient descent to match the Q-values predicted by the DQN and the expected
Q-values from the Bellman equation, $r_i + \gamma max_aQ(s_{i+1}, a; \theta)$.
Samples are randomly selected from the experience memory to update the
parameters of the DQN by minimizing the loss function:
\begin{equation}
    \mathbb{L}(\theta) = (r+ max_{a'}Q(s',a')-Q(s,a))^2
\end{equation}    
The training procedure is repeated with the incoming instances. We conduct a
significance test to decide whether the training episode should be terminated.
In the significance test, we calculate the performance difference between a
series of consecutive actions. If the performance difference of the tagger is
not significant, we terminate the training episode and restart the training with
a new episode.

%may add an algorithm here
\begin{algorithm}[!t] 
\caption{Self training for in-domain tagging}
\label{alg:indomain}
\KwIn{unlabeled data $U$, dev set $D$, test set $T$;}
\KwOut{A self-training tagger;}
%\Begin{
    randomly select a subset $init$ from $D$\;
    $ds \leftarrow init$\; 
    //training DQN\\
    \While {$episode < 10000$} { 
        $tagger\leftarrow train(ds)$\;
        $performance \leftarrow test(tagger, D)$\;
        \While {$significant(performance)$}{
             $U \leftarrow U \backslash {x} $\; 
             $qvalue \leftarrow DQN(x)$\;
             \If{ $argmax(qvalue) == 1$} {
                 $y \leftarrow tag(tagger, x)$\;
                 $ds \leftarrow ds\cup (x, y)$ \;
                 $tagger \leftarrow train(ds)$\;
                 $reward \leftarrow test(tagger, D) - performance$\;
                 $update(DQN, reward)$\;
             }    
        }

        $episode \leftarrow episode +1$ \;
    }   

    //train the final tagger\\
    $ds \leftarrow init$\; 
    $tagger \leftarrow train(ds)$\;
    \While {$has(budget)$} { 
        $U \leftarrow U \backslash {x} $\;
        $qvalue \leftarrow DQN(x)$\;
        \If {$argmax(qvalue) == 1$} {
             $y \leftarrow tag(tagger,x)$\;
             $ds \leftarrow ds \cup (x, y)$ \;
             $tagger\leftarrow train(ds)$\;
        }    
    }
%}    
\end{algorithm}


\subsection{Tasks}

The deep reinforcement learning neural network for self-learning (denoted as
DQN) can be used for various application scenarios where gold labels are not
available and the efforts to annotate the labels are expensive. In this section,
we illustrate two application scenarios.

\textbf{Self Training for Zero-shot In-domain Tagging}
In this scenario, the gold label of the training dataset is not available. Only
a small development and test dataset is annotated with gold labels. In this
scenario, we need to apply a self-learning approach to train a tagger that can
be used to tag the unlabeled instances with an acceptable performance.

Algorithm~\ref{alg:indomain} illustrates our solution. In order to learn the
self-learning approach for this scenario, we randomly select a small number of
instances with gold labels from the development dataset. These instances are
then used to initialize the tagger for the self-training. Whenever an unlabeled instance is selected and added to the training set to retrain the tagger, the
performance difference of the tagger on the remaining development data set is calculated
as reward of the action. The reward is regarded as a feedback of the action and
is used to update the parameters of the DQN neural network. The DQN neural
network is self-trained for a given number of episodes. Once the training of the
DQN is finished, we use it to select unlabeled instances from the training
dataset and train the tagger based on those selected unlabeled instances
(together with their predicted labels).

\textbf{Self Training for Domain Adaptation}

In this scenario, we have a source domain with a training set with gold
labels, but the target domain has only a small development set equipped with
gold labels. In this scenario, we need to apply a self-learning approach to
transfer the knowledge learned from the source domain to the target domain. 

The algorithm is similar to Algorithm~\ref{alg:indomain}. The main difference is that
we train the tagger using the training dataset from the source domain. 
%The purpose is to transfer the knowledge from the source domain to the target domain. 
%Then, this tagger is set as the initialized tagger to train the DQN
%using the unlabeled data from the target domain. If the DQN selects an unlabeled
%instance, the tagger is used to tag this instance. This instance and the
%predicted labels are then added to the training set to retrain the tagger.
%Similarly, the performance difference is calculated as the feedback of the
%action and used to update the parameters of the DQN neural network. 
The DQN neural network is also self-trained for a given number of episodes. Once the training of the DQN is finished, we use the DQN to select unlabeled instances from the
target domain. These selected instances are added together with the training
dataset from the source domain to train the tagger for the target domain.

%may add an algorithm here


==> method3.tex <==
\section{Self-training}\label{sec:slmethod}
%formalize the problem as a self-learning problem
As explained in Section~\ref{section:intro}, we investigate how to learn a
self-training approach that can be applied to multiple scenarios where the gold labels are not available and the efforts for human to annotate the labels are expensive. Our goal is to retrieve useful information from the massive unlabeled dataset to improve the training performance.

In traditional self-training framework (Algorithm~\ref{alg:tsl}), a tagger is first initialized using a set of 
instances with gold labels. Then, this tagger is used to tag a set of unlabeled data, and the tagging confidence for each unlabeled
instance is evaluated. The automatically labeled instances  with the highest confidence is added to the
training set. The tagger is retrained using the updated training dataset and used to tag and select the unlabeled instances from the remaining dataset. This procedure is repeated until a given number of instances are selected and added to the training dataset. 

How to measure the confidence of a tagging is crucial to a self-training
approach. Traditional self-training approach usually requires human efforts to design specific confidence metrics based on the heuristics and application
scenarios. This, however, is challenging and the effectiveness of the solution may depend on many factors, which however is not well investigated yet. We propose to learn a self-training strategy automatically. 

%In traditional self-learning framework, the selection of an unlabeled instance
%can be regarded as a decision process, in the sense that the learning strategy
%decides whether an unlabeled instance is added to the training dataset or not in
%each step. Also, the selection of an unlabeled instance in current step depends
%on the selection of an unlabeled instance in the previous step, since the tagger is
%retrained once an unlabeled instance is selected and added to the training
%dataset. Therefore, a self-learning procedure can be regarded as a function that
%takes the current state of the self-learning framework as input and generates
%the output indicating whether an unlabeled instance is selected or not. In
%traditional self-learning approaches, this function is usually designed manually
%with some heuristics. In this paper, we propose to learn this function
%automatically using a deep reinforcement learning network. 

\begin{algorithm}[!t] 
\caption{Self-training}
\label{alg:tsl}
\KwIn{dataset train $T$, dev $D$, budget; unlabeled data $U$}
randomly shuffle $U$; $i \leftarrow 0$\;
\While{$i < budget$ and $U$ is not empty}{
    $tagger\leftarrow train(T, D)$\;
    $tag(tagger,U)$ \;
    $x \leftarrow select(U)| \max_{x}{\it confidence}(y)$\;
    $T \leftarrow T \cup (x, y)$\;
    $U \leftarrow U \backslash (x, y)$\;
    $i \leftarrow i + 1$\;
}
\KwOut{$tagger$;}
\end{algorithm}

\section{Learning how to self-train}\label{sec:dqnmethod}

%In a self-training framework, the selection of an unlabeled instance
%can be regarded as a decision process, in the sense that the learning strategy
%decides whether an unlabeled instance is added to the training dataset or not in
%each step. Therefore, a self-training procedure can be regarded as a function that
%takes the current state of the self-learning framework as input and generates
%the output indicating whether an unlabeled instance is selected or not. In
%traditional self-training approaches, this function is usually designed manually
%with some heuristics. In this section, we propose to learn this function
%automatically using a deep reinforcement learning neural network. 

In order to learn a self-training function automatically, we design a deep
reinforcement learning neural network to optimize the function parameters based on the
feedback from the training. 
To formalize the self-training function easily, we
adopt a stream-based strategy. That is, the unlabeled training dataset is
regarded as a stream of instances. For every arriving unlabeled instance, the
self-training function generates an output indicating whether this instance is
selected or not. Given a stream of unlabeled dataset, our goal is to train the
function that can make the decision automatically with a good performance via
reinforcement learning.

\begin{figure*}[!t] 
\centering
\includegraphics[width=0.7\linewidth]{qnet3.png}
\caption{The neural network for Q-function}
\label{fig:dqn}
\end{figure*}

%an introduction to reinforcement learning 
{\bf Training Goal} Reinforcement learning has been well adopted to learn a policy function in many
applications scenarios. In this paper, similar to the setting in
~\cite{fang2017activelearning}, we adopt the deep Q-learning approach~\cite{nature14} as our
learning framework (denoted as DQN). In this learning framework, the policy
function $\pi$ is defined via a Q-function: $Q^{\pi}(s,a)\to R$, where $s$ is
the current state of learning framework, $a$ is the action, and $R$ is the
reward of the framework when taking action $a$ from the current state $s$. The
training of the policy function $\pi$ is to find the parameters that can
maximize the reward of the each action in every state. This is done by
iteratively updating $Q^{\pi}(s,a)$ using the rewards obtained from the
sequence of actions during the training, based on the Bellman equation defined
as follows: 
\begin{equation} 
    Q^{\pi}(s,a) = \mathbb{E}[R_i|s_i=s, a_i=a, \pi]
\end{equation} 
where $R_i = \sum_{t=i}^T \gamma^{t-i} r_t$ is the discounted
future rewards and $\gamma\in[0,1]$ is the discounting rate. 



\subsection{Model Structure}

We follow the setting in the deep Q-learning approach~\cite{nature14} to
calculate the expected $Q$ value to update the parameters. We implement the
Q-function using a three-layered neural network, as shown in Fig.~\ref{fig:dqn}.

%state
The input layer represents the state of the learning framework. We adopt a
similar approach proposed by \newcite{fang2017activelearning} to define the state of the
framework. In particular, a state $s$ consists of three elements ($h_s$, $h_c$, $h_p$),
where $h_s$ is the content representation of the arriving instance, $h_c$ is the
confidence of tagging the instance using the tagger, and $h_p$ is the marginals
of the prediction for this instance.

As shown in Fig.~\ref{fig:dqn}, to represent the content of an arriving
instance, a convolutional neural network (CNN) with 384 filters are designed, with the convolution size being (3, 4, 5), and 128 filters 
for each size, respectively. Each filter uses a linear transformation with a
rectified linear unit activation function. The input to the CNN is the
concatenated word embedding of the instance via looking up a pre-trained word
embedding. These filters are used to extract the features of the instance
contents. The filter outputs are then merged using a max-pooling operation to
yield a hidden state $h_s$, a vector of size 384 that represents the
content of this instance.

The confidence of the tagger for an instance $h_c$ is defined based on the most
probable label sequence for this instance. In this paper, we adopt in the
experiment a CRF tagger and its confidence value can be taken directly from the
CRF tagger. This value can be also defined and measured for different taggers. 

The marginals of the prediction for an instance is also calculated based on a
CNN. The labels of the arriving instance are predicted using the tagger and 20
filters with a size of 3 are designed to extract the features in the prediction.
These feature maps are then sub-sampled with mean pooling to capture the average
uncertainty in each filter. The final hidden layer $h_p$ is used to represent
the predictive marginals. 

%action
The three elements of the state $s=(h_s, h_c, h_p)$ are then used to calculate the
second layer with a rectified linear unit activation function. This hidden layer
is designed as a vector of size 256. Then it is used to calculate expected
Q-value in the output layer, a vector of size 2, indicating whether the
instance should be selected or not. If an instance is selected, the predicted
labels of the sentences together with this sentence are added to the training
set to retrain the tagger.

{\bf Reward} To train this neural network via reinforcement learning, we need to define the
reward for each action. If an instance is not selected, then the reward is set
to 0; otherwise, the reward of this action is defined as the performance
difference of the tagger after the instance is added to the training set. 

%budget for each episode (significance test) 

Following the approach of \newcite{nature14}, we train the DQN using an experience
replay mechanism. The current state, its actions and corresponding rewards are
recorded in a memory. The parameters of DQN are learned using stochastic
gradient descent to match the Q-values predicted by the DQN and the expected
Q-values from the Bellman equation, $r_i + \gamma max_aQ(s_{i+1}, a; \theta)$.
Samples are randomly selected from the experience memory to update the
parameters of the DQN by minimizing the loss function:
\begin{equation}
    \mathbb{L}(\theta) = (r+ max_{a'}Q(s',a')-Q(s,a))^2
\end{equation}    
The training procedure is repeated with the incoming instances. We conduct a
significance test to decide whether the training episode should be terminated.
In the significance test, we calculate the performance difference between a
series of consecutive actions. If the performance difference of the tagger is
not significant, we terminate the training episode and restart the training with
a new episode.

%may add an algorithm here
\begin{algorithm}[!t] 
\caption{DQN-based self-training for zero-shot in-domain tagging}
\label{alg:indomain}
\KwIn{unlabeled data $U$, dev set $D$;}
\KwOut{$tagger$;}
%\Begin{
    randomly select a subset $init$ from $D$\;
    $ds \leftarrow init$\; 
    //train the DQN, c.f. Algorithm~\ref{alg:dqn}\\
    $DQN \leftarrow selftrain(U, D, ds)$ \;
    //train the final tagger\\
    $ds \leftarrow init$; $tagger \leftarrow train(ds)$\;
    \While {$has(budget)$} { 
        $x\leftarrow$ a random instance from $U$\;
        $U \leftarrow U \backslash {x} $\;
        $qvalue \leftarrow DQN(x, tagger)$\;
        \If {$argmax(qvalue) == 1$} {
             $y \leftarrow tag(tagger,x)$\;
             $ds \leftarrow ds \cup (x, y)$ \;
             $tagger\leftarrow train(ds)$\;
        }    
    }
%}    
\end{algorithm}

\begin{algorithm}[!t] 
\caption{Self-train a DQN}
\label{alg:dqn}
\KwIn{unlabeled data $U$, dev set $D$, initial set $init$;}
\KwOut{$DQN$;}
    $ds \leftarrow init$\;
    \While {$episode < 10000$} { 
        $tagger\leftarrow train(ds)$\;
        $score \leftarrow test(tagger, D)$\;
        
        \While {$significant(score)$}{
             $x\leftarrow$ a random instance from $U$\;
             $U \leftarrow U \backslash {x} $; $reward \leftarrow 0$\;
             $qvalue \leftarrow DQN(x, tagger)$\;
             \If{ $argmax(qvalue) == 1$} {
                 $y \leftarrow tag(tagger, x)$\;
                 $ds \leftarrow ds\cup (x, y)$ \;
                 $tagger \leftarrow train(ds)$\;
                 $newscore \leftarrow test(tagger, D)$\;
                 $reward \leftarrow newscore - score$\;
                 $score\leftarrow newscore$\;
             }
             train $DQN(x, tagger, reward)$\;
        }
        $episode \leftarrow episode +1$ \;
    }   
\end{algorithm}
\subsection{Tasks}
The deep reinforcement learning neural network for self-learning (denoted as
DQN) can be used for various application scenarios where gold labels are not
available and the efforts to annotate the labels are expensive. In this section,
we illustrate two application scenarios.

\textbf{Self Training for Zero-shot In-domain Tagging}
In this scenario, the gold label of the training dataset is not available. Only
a small development and test dataset is annotated with gold labels. In this
scenario, we need to apply a self-learning approach to train a tagger that can
be used to tag the unlabeled instances with an acceptable performance.

Algorithm~\ref{alg:indomain} illustrates our solution. In order to learn the
self-learning approach for this scenario, we randomly select a small number of
instances with gold labels from the development dataset. These instances are
then used to initialize the tagger for the self-training of the DQN (c.f., Algorithm~\ref{alg:dqn}). Whenever an unlabeled instance is selected and added to the training set to retrain the tagger, the
performance difference of the tagger on the remaining development data set is calculated
as reward of the action. The reward is regarded as a feedback of the action and
is used to update the parameters of the DQN neural network. The DQN neural
network is self-trained for a given number of episodes. Once the training of the
DQN is finished, we use it to select unlabeled instances from the training
dataset and train the tagger based on those selected unlabeled instances
(together with their predicted labels).

\textbf{Self Training for Domain Adaptation}

\begin{algorithm}[!t] 
\caption{DQN-based self-training for domain adaptation}
\label{alg:crossdomain}
\KwIn{unlabeled data $U$, dev set $D$; source data $source$}
\KwOut{$tagger$;}
%\Begin{
    $ds \leftarrow source$\; 
    //train the DQN, c.f. Algorithm~\ref{alg:dqn}\\
    $DQN \leftarrow selftrain(U, D, ds)$ \;

    //train the final tagger\\
    $ds \leftarrow source$; $tagger \leftarrow train(ds)$\;
    \While {$has(budget)$} { 
        $x\leftarrow$ a random instance from $U$\;
        $U \leftarrow U \backslash {x} $\;
        $qvalue \leftarrow DQN(x, tagger)$\;
        \If {$argmax(qvalue) == 1$} {
             $y \leftarrow tag(tagger,x)$\;
             $ds \leftarrow ds \cup (x, y)$ \;
             $tagger\leftarrow train(ds)$\;
        }    
    }
%}    
\end{algorithm}

In this scenario, we have a source domain with a training set with gold
labels, but the target domain has only a small development set equipped with
gold labels. In this scenario, we need to apply a self-learning approach to
transfer the knowledge learned from the source domain to the target domain, as depicted in Algorithm~\ref{alg:crossdomain}. 

Algorithm~\ref{alg:crossdomain} is similar to Algorithm~\ref{alg:indomain}. The main difference is that
we train the baseline tagger using the training dataset from the source domain. 
%The purpose is to transfer the knowledge from the source domain to the target domain. 
%Then, this tagger is set as the initialized tagger to train the DQN
%using the unlabeled data from the target domain. If the DQN selects an unlabeled
%instance, the tagger is used to tag this instance. This instance and the
%predicted labels are then added to the training set to retrain the tagger.
%Similarly, the performance difference is calculated as the feedback of the
%action and used to update the parameters of the DQN neural network. 
The DQN neural network is also self-trained for a given number of episodes (c.f., Algorithm~\ref{alg:dqn}). Once the training of the DQN is finished, we use the DQN and the baseline model trained from source domain to select unlabeled instances from the
target domain. These selected instances are added together with the training
dataset from the source domain to train the tagger for the target domain.

%may add an algorithm here


==> method4.tex <==
\section{Self-training}\label{sec:slmethod}
%formalize the problem as a self-learning problem
As explained in Section~\ref{section:intro}, we investigate how to learn a
self-training approach that can be applied to multiple scenarios where the gold labels are not available and the efforts for human to annotate the labels are expensive. Our goal is to retrieve useful information from the massive unlabeled dataset to improve the training performance.

In traditional self-training framework (Algorithm~\ref{alg:tsl}), a tagger is first initialized using a set of 
instances with gold labels. Then, this tagger is used to tag a set of unlabeled data, and the tagging confidence for each unlabeled
instance is evaluated. The automatically labeled instances  with the highest confidence is added to the
training set. The tagger is retrained using the updated training dataset and used to tag and select the unlabeled instances from the remaining dataset. This procedure is repeated until a given number of instances are selected and added to the training dataset. 

How to measure the confidence of a tagging is crucial to a self-training
approach. Traditional self-training approach usually requires human efforts to design specific confidence metrics based on the heuristics and application
scenarios. This, however, is challenging and the effectiveness of the solution may depend on many factors, which however is not well investigated yet. We propose to learn a self-training strategy automatically. 

%In traditional self-learning framework, the selection of an unlabeled instance
%can be regarded as a decision process, in the sense that the learning strategy
%decides whether an unlabeled instance is added to the training dataset or not in
%each step. Also, the selection of an unlabeled instance in current step depends
%on the selection of an unlabeled instance in the previous step, since the tagger is
%retrained once an unlabeled instance is selected and added to the training
%dataset. Therefore, a self-learning procedure can be regarded as a function that
%takes the current state of the self-learning framework as input and generates
%the output indicating whether an unlabeled instance is selected or not. In
%traditional self-learning approaches, this function is usually designed manually
%with some heuristics. In this paper, we propose to learn this function
%automatically using a deep reinforcement learning network. 

\begin{algorithm}[!t] 
\caption{Self-training}
\label{alg:tsl}
\KwIn{dataset train $T$, dev $D$, budget; unlabeled data $U$}
randomly shuffle $U$; $i \leftarrow 0$\;
\While{$i < budget$ and $U$ is not empty}{
    $tagger\leftarrow train(T, D)$\;
    $tag(tagger,U)$ \;
    $x \leftarrow select(U)| \max_{x}{\it confidence}(y)$\;
    $T \leftarrow T \cup (x, y)$\;
    $U \leftarrow U \backslash (x, y)$\;
    $i \leftarrow i + 1$\;
}
\KwOut{$tagger$;}
\end{algorithm}

\section{Learning how to self-train}\label{sec:dqnmethod}

%In a self-training framework, the selection of an unlabeled instance
%can be regarded as a decision process, in the sense that the learning strategy
%decides whether an unlabeled instance is added to the training dataset or not in
%each step. Therefore, a self-training procedure can be regarded as a function that
%takes the current state of the self-learning framework as input and generates
%the output indicating whether an unlabeled instance is selected or not. In
%traditional self-training approaches, this function is usually designed manually
%with some heuristics. In this section, we propose to learn this function
%automatically using a deep reinforcement learning neural network. 

In order to learn a self-training function automatically, we design a deep
reinforcement learning neural network to optimize the function parameters based on 
feedback from a set of development data.  
To formalize the self-training function easily, we
adopt a stream-based strategy. That is, the unlabeled training dataset is
regarded as a stream of instances. For every arriving unlabeled instance, the
self-training function generates an output indicating whether this instance is
selected or not. Given a stream of unlabeled dataset, our goal is to train the
function that can make the decision automatically with a good performance via
reinforcement learning.

\begin{figure*}[!t] 
\centering
\includegraphics[width=0.7\linewidth]{qnet3.png}
\caption{The neural network for Q-function}
\label{fig:dqn}
\end{figure*}

%an introduction to reinforcement learning 
\subsection{DQN-based self-training}

\begin{algorithm}[!t] 
\caption{DQN-based self-training}
\label{alg:indomain}
\KwIn{dataset train T, dev set $D$, unlabeled data $U$,  budget;}
\KwOut{$tagger$;}
%\Begin{
    //train the DQN, c.f. Algorithm~\ref{alg:dqn}\\
    $DQN \leftarrow selftrain(U, D, T)$ \;
    $tagger \leftarrow train(T, D)$; $i \leftarrow 0$\;
    \While {$i<budget$ and $U$ is not empty} { 
        $x\leftarrow$ a random instance from $U$\;
        $U \leftarrow U \backslash {x} $\;
        $qvalue \leftarrow DQN(x, tagger)$\;
        \If {$argmax(qvalue) == 1$} {
             $y \leftarrow tag(tagger,x)$\;
             $T \leftarrow T \cup (x, y)$ \;
             $tagger\leftarrow train(T, D)$\;
             $i \leftarrow i+1$\;
        }    
    }
%}    
\end{algorithm}

Pseudo code for DQN-based self-training is shown in Algorithm \ref{alg:indomain}. Compared with Algorithm \ref{alg:tsl}, Algorithm \ref{alg:indomain} is different in three aspects. First, when making a choice, Algorithm \ref{alg:indomain} randomly access a unlabeled instance, while Algorithm \ref{alg:tsl} needs to visit a batch of instances. Second, Algorithm \ref{alg:tsl} directly uses model confidence score to choose instance, while Algorithm \ref{alg:indomain} train a DQN to learn a Q-function ($qvalue$),  approximating the confidence score automatically. Third, Algorithm \ref{alg:tsl} select one instance for each iteration, while Algorithm \ref{alg:indomain} makes a choice only when the rejection score ($qvalue[0]$) is less than the acceptance score ($qvalue[1]$). 

{\bf Training Goal.} Reinforcement learning has been well adopted to learn a policy function in many
applications scenarios. In this paper, similar to the setting in
~\cite{fang2017activelearning}, we adopt the deep Q-learning approach~\cite{nature14} as our
learning framework (denoted as DQN). In this learning framework, the policy
function $\pi$ is defined via a Q-function: $Q^{\pi}(s,a)\to R$, where $s$ is
the current state of learning framework, $a$ is the action, and $R$ is the
reward of the framework when taking action $a$ from the current state $s$. The
training of the policy function $\pi$ is to find the parameters that can
maximize the reward of the each action in every state. This is done by
iteratively updating $Q^{\pi}(s,a)$ using the rewards obtained from the
sequence of actions during the training, based on the Bellman equation defined
as follows: 
\begin{equation} 
    Q^{\pi}(s,a) = \mathbb{E}[R_i|s_i=s, a_i=a, \pi]
\end{equation} 
where $R_i = \sum_{t=i}^T \gamma^{t-i} r_t$ is the discounted
future rewards and $\gamma\in[0,1]$ is the discounting rate. 



\subsection{Model Structure}

We follow the setting in the deep Q-learning approach~\cite{nature14} to
calculate the expected $Q$ value to update the parameters. We implement the
Q-function using a three-layered neural network, as shown in Fig.~\ref{fig:dqn}.

%state
The input layer represents the state of the learning framework. We adopt a
similar approach proposed by \newcite{fang2017activelearning} to define the state of the
framework. In particular, a state $s$ consists of three elements ($h_s$, $h_c$, $h_p$),
where $h_s$ is the content representation of the arriving instance, $h_c$ is the
confidence of tagging the instance using the tagger, and $h_p$ is the marginals
of the prediction for this instance.

As shown in Fig.~\ref{fig:dqn}, to represent the content of an arriving
instance, a convolutional neural network (CNN) with 384 filters are designed, with the convolution size being (3, 4, 5), and 128 filters 
for each size, respectively. Each filter uses a linear transformation with a
rectified linear unit activation function. The input to the CNN is the
concatenated word embedding of the instance via looking up a pre-trained word
embedding. These filters are used to extract the features of the instance
contents. The filter outputs are then merged using a max-pooling operation to
yield a hidden state $h_s$, a vector of size 384 that represents the
content of this instance.

The confidence of the tagger for an instance $h_c$ is defined based on the most
probable label sequence for this instance. In this paper, we adopt in the
experiment a CRF tagger and its confidence value can be taken directly from the
CRF tagger. This value can be also defined and measured for different taggers. 

The marginals of the prediction for an instance is also calculated based on a
CNN. The labels of the arriving instance are predicted using the tagger and 20
filters with a size of 3 are designed to extract the features in the prediction.
These feature maps are then sub-sampled with mean pooling to capture the average
uncertainty in each filter. The final hidden layer $h_p$ is used to represent
the predictive marginals. 

%action
The three elements of the state $s=(h_s, h_c, h_p)$ are then used to calculate the
second layer with a rectified linear unit activation function. This hidden layer
is designed as a vector of size 256. Then it is used to calculate expected
Q-value in the output layer, a vector of size 2, indicating whether the
instance should be selected or not. If an instance is selected, the predicted
labels of the sentences together with this sentence are added to the training
set to retrain the tagger.

\subsection{Training DQN}

{\bf Reward.} To train this neural network via reinforcement learning, we need to define the
reward for each action. If an instance is not selected, then the reward is set
to 0; otherwise, the reward of this action is defined as the performance
difference of the tagger after the instance is added to the training set. 

%budget for each episode (significance test) 

Following the approach of \newcite{nature14}, we train the DQN using an experience
replay mechanism. The current state, its actions and corresponding rewards are
recorded in a memory. The parameters of DQN are learned using stochastic
gradient descent to match the Q-values predicted by the DQN and the expected
Q-values from the Bellman equation, $r_i + \gamma max_aQ(s_{i+1}, a; \theta)$.
Samples are randomly selected from the experience memory to update the
parameters of the DQN by minimizing the loss function:
\begin{equation}
    \mathbb{L}(\theta) = (r+ max_{a'}Q(s',a')-Q(s,a))^2
\end{equation}    
The training procedure is repeated with the incoming instances. We conduct a
significance test to decide whether the training episode should be terminated.
In the significance test, we calculate the performance difference between a
series of consecutive actions. If the performance difference of the tagger is
not significant, we terminate the training episode and restart the training with
a new episode.

%may add an algorithm here
\begin{algorithm}[!t] 
\caption{Self-train a DQN}
\label{alg:dqn}
\KwIn{unlabeled data $U$, dev set $D$, initial set $init$;}
\KwOut{$DQN$;}
    $T \leftarrow init$\;
    \While {$episode < 10000$} { 
        $tagger\leftarrow train(T)$\;
        $score \leftarrow test(tagger, D)$\;
        
        \While {$significant(score)$}{
             $x\leftarrow$ a random instance from $U$\;
             $U \leftarrow U \backslash {x} $; $reward \leftarrow 0$\;
             $qvalue \leftarrow DQN(x, tagger)$\;
             \If{ $argmax(qvalue) == 1$} {
                 $y \leftarrow tag(tagger, x)$\;
                 $T \leftarrow T\cup (x, y)$ \;
                 $tagger \leftarrow train(T)$\;
                 $newscore \leftarrow test(tagger, D)$\;
                 $reward \leftarrow newscore - score$\;
                 $score\leftarrow newscore$\;
             }
             train $DQN(x, tagger, reward)$\;
        }
        $episode \leftarrow episode +1$ \;
    }   
\end{algorithm}

{\bf Algorithm.} Algorithm \ref{alg:dqn} shows the pseudo  code for DQN training. First, A initial set $init$ is 
 used to train the baseline $tagger$. 
 Then, a random initialized DQN evaluate the Q-value of an instance sampled from the unlabeled set $U$. 
 Then when the corresponding Q-value of acceptance is larger than that of rejection, the instance is selected. 
 This raw instance together with its predicted labels is added to the training set. A new tagger is trained using the augmented training set. 
 When a selection happens, the performance difference between the new tagger and the old tagger on the development data set is calculated
as reward of the action. The reward is regarded as a feedback of the action and
is used to update the parameters of the DQN neural network . The DQN neural
network is self-trained for a given number of episodes. Once the performance on the development set is stable, the training of the
DQN stops.

\section{Tasks}
The deep reinforcement learning neural network for self-learning can be used for various application scenarios where gold labels are not
available and the efforts to annotate the labels are expensive. In this section,
we illustrate two application scenarios.

\textbf{Self Training for Zero-shot In-domain Tagging.} In this scenario, the gold label of the training dataset is not available. Only
a small development and test dataset is annotated with gold labels.  We need to apply a self-learning approach to train a tagger that can
be used to tag the unlabeled instances with an acceptable performance.

This solution is the same as Algorithm~\ref{alg:indomain}. In order to learn the
self-learning approach for this scenario, we randomly select a small number of
instances with gold labels from the development dataset. This equals to setting the training set $T$ in Algorithm \ref{alg:indomain} to be a random subset $init$ from the develpoment set. 
These instances are
then used to initialize the tagger ($tagger \leftarrow train(T)$) for the self-training of the DQN (c.f., Algorithm~\ref{alg:dqn}). Once the training of the
DQN is finished, we use it to select unlabeled instances from the training
dataset and train the tagger based on those selected unlabeled instances
(together with their predicted labels).

\textbf{Self Training for Domain Adaptation.} In this scenario, we have a source domain with a training set with gold
labels, but the target domain has only a small development set equipped with
gold labels. We need to apply a self-learning approach to
transfer the knowledge learned from the source domain to the target domain. 

We train the baseline tagger using the training dataset from the source domain. Corresponding to Algorithm \ref{alg:indomain}, the training set $T$ means the labeled training set in source domain. 
%The purpose is to transfer the knowledge from the source domain to the target domain. 
%Then, this tagger is set as the initialized tagger to train the DQN
%using the unlabeled data from the target domain. If the DQN selects an unlabeled
%instance, the tagger is used to tag this instance. This instance and the
%predicted labels are then added to the training set to retrain the tagger.
%Similarly, the performance difference is calculated as the feedback of the
%action and used to update the parameters of the DQN neural network. 
The DQN neural network is also self-trained for a given number of episodes (c.f., Algorithm~\ref{alg:dqn}). Once the training of the DQN is finished, we use the DQN and the baseline model trained from source domain to select unlabeled instances from the
target domain. These selected instances are added together with the training
dataset from the source domain to train the tagger for the target domain.

%may add an algorithm here


==> relatedwork.tex <==



\section{Related Work}\label{sec:RW}
%literature review logic
%1)one or two sentences to introduce the techniques
%2)How existing work addresses the issues in this areas
%3)The limitation of existing work
%4)The difference between existing work and ours
 In this section, we briefly review previous work on
reinforcement learning, self-training and domain adaptation in the NLP area.
\textbf{Self Training} is a simple semi-supervised algorithm that has shown some
surprising success in parsing ~\cite{McClosky2006parsing,mcclosky2008self,Huang2009latentpcfg,Sagae2010parseradaptation},
part of speech tagging~\cite{wang2007semi,huang2009bigramhmm,qi2009semi}, named entity recognition~\cite{kozareva2005self,liu2013ner}, 
sentiment classification~\cite{van2016predicting,drury2011guidedself,liu2013reserved}, and other NLP tasks. 


The performance of the self-training algorithms strongly depends on the
selected newly-labeled data at each iteration of the training procedure. Most
of the current self-training approaches set up a threshold and treat a set of
unlabeled examples as the high-confident prediction if its prediction is above
the pre-defined threshold value. Such selection metric may not provide a
reliable selection~\cite{Chenmm2011nips}. 

Some researchers explore extra metrics as an auxiliary measurement to evaluate
instances from unlabeled data. For example, 
\newcite{Ardehaly2016domainadaptation} use coefficients learned from the model on the
source domain as a selection metric when applying self training in the target for
hierarchical multi-label classification task and report a positive effect. 
 \newcite{Jason2011emnlp} propose to produce a ranked list of n-best predicted parses 
 and select the one yields the best external evaluation scored on the downstream external task (i.e., machine translation).
\newcite{rosenberg2005semi} examine a few selection metrics for object detection
task, and show that detector-independent metric outperforms the more
intuitive confidence metric. Various pseudo-labeled example selection
strategies \cite{medlock2007weakly,daume2008cross} have been proposed.

\newcite{zhou2012self} explore a guided
search algorithm to find
informative unlabeled data subsets in the self-training process. The
experiment results demonstrate that the proposed algorithm is in general more
reliable and more effective than the standard self-training algorithm.  But
these heuristic choices require careful parameter tuning and domain specific
information.

Most recently, \newcite{Levati2017tree} propose an algorithm to
automatically identify an appropriate threshold from a candidate list for the
reliability of predictions. The automatic selected threshold is to be used in
the next iteration of self-training procedure. They score each candidate
threshold by evaluating whether the mean of the out of bag error between the
examples with reliability score greater than the considered threshold is
significantly different from the mean of the out of bag error of all the
examples.  


Self-training techniques have also been explored for domain adaptation by some
researchers. For example, \newcite{Ardehaly2016domainadaptation} use 
self-training process to adapt the label proportion model from the source
domain to the target domain.  \newcite{chattopadhyay2012multisource} generate 
pseudo-labels for the target data. \newcite{daume2008cross} propose a self
training method in which several models are trained on the same dataset, and
only unlabeled instances that satisfy the cross task knowledge constraints are used in the self training process.

\newcite{He:2011featureadaptation} derive  a set of self-learned and domain-specific features that are
related to the distribution of the target classes for sentiment analysis task. 
Such self-learned features are then used to train another classifier 
by constraining the model’s predictions on unlabeled instances.

Note that although there have been many studies on how to apply self-training to
NLP tasks, all the work design the self-training strategy manually based on the
heuristics of the NLP tasks. This makes it difficult to apply these approaches
to a different NLP task or a different application scenario. Differently, we
propose to design a general self-training approach by learning the self-training
strategy automatically. In this way, our solution can be easily applied to
different application domains.

%{\bf Deep reinforcement learning for NLP} 
There are also some relevant works on reinforcement learning for natural language
processing, such as machine translation \cite{grissom2014don,guo2015generating,gu2016learning,xia2016dual,bahdanau2016actor}, dialog systems \cite{li2016dialogue,su2016continuously}, sentence simplification \cite{zhang2017sentence,narayan2017split}, co-reference resolution \cite{clark2016deep} and latent structure induction \cite{Yogatama2016word2sentence,lei2016rationale}. 
In particular, \newcite{guo2015generating} propose a deep Q-network model for text generation in sequence-to-sequence models. \newcite{fang2017activelearning} leverage  reinforcement learning for active learning, where a deep Q-network is used to learn the query policy for the active learners.  
%. For example, \newcite{su2016continuously} combined reinforcement learning with
%neural generation on tasks with real users, showing that reinforcement learning
%improves dialogue performance.\newcite{clark2016deep} applied reinforcement
%learning to directly optimize a neural mention-ranking model for co-reference
%evaluation metrics. xxx~\cite{} investigate knowledge transferring from source
%domain to target domain through.... 
%\newcite{Yogatama2016word2sentence} used reinforcement learning to induce implicit syntax structures via auxiliary tasks. \newcite{lei2016rationale} extracted rationales for sentiment prediction and question retrieval tasks. 
However, to the best of our knowledge, there has been no previous attempts to
embed self-training to deep reinforcement learning framework. 
The active learning work of \newcite{fang2017activelearning} is most similar to us. However, different from active learning which need to query human experts or oracle to provide gold labels,  
self-training associates instances with automatic prediction label. This makes our work substantially different from the work of \newcite{fang2017activelearning}. 





%active learning (\cite{fang2017activelearning})



==> relatedwork3.tex <==



\section{Related Work}\label{sec:RW}

%Scarcity of annotated data has motivated the research into techniques capable
%of exploiting unlabeled data, e.g., domain adaptation, semi-supervised and
%unsupervised learning. 
%literature review logic
%1)one or two sentences to introduce the techniques
%2)How existing work addresses the issues in this areas
%3)The limitation of existing work
%4)The difference between existing work and ours
In this section, we briefly review previous work on
reinforcement learning, self-training and domain adaptation in the NLP area.
\textbf{Self Training} is a simple semi-supervised algorithm that has shown some
surprising success in parsing ~\cite{McClosky2006parsing,mcclosky2008self,Huang2009latentpcfg,Sagae2010parseradaptation},
part of speech tagging~\cite{wang2007semi,huang2009bigramhmm,qi2009semi}, named entity recognition~\cite{kozareva2005self,liu2013ner}, 
sentiment classification~\cite{van2016predicting,drury2011guidedself,liu2013reserved}, and other NLP tasks. 


The performance of the self-training algorithms strongly depends on the
selected newly-labeled data at each iteration of the training procedure. Most
of the current self-training approaches set up a threshold and treat a set of
unlabeled examples as the high-confident prediction if its prediction is above
the pre-defined threshold value. Such selection metric may not provide a
reliable selection~\cite{Chenmm2011nips}. 

Some researchers explore extra metrics as an auxiliary measurement to evaluate
instances from unlabeled data. For example, 
\newcite{Ardehaly2016domainadaptation} used coefficients learned from the model on the
source domain as a selection metric when applying self training in the target for
hierarchical multi-label classification task and report a positive effect. 
 \newcite{Jason2011emnlp} proposed to produce a ranked list of n-best predicted parses 
 and selected the one yields the best external evaluation scored on the downstream external task (i.e., machine translation).
\newcite{rosenberg2005semi} examined a few selection metrics for object detection
task, and showed that detector-independent metric outperforms the more
intuitive confidence metric. Various pseudo-labeled example selection
strategies \cite{medlock2007weakly,daume2008cross} have been proposed.

\newcite{zhou2012self} explore a guided search algorithm to find informative unlabeled data subsets in the self-training process. The experimental results demonstrate that the proposed algorithm is in general more reliable and more effective than the standard self-training algorithm. But these heuristic choices require careful parameter tuning and domain specific information.

Most recently, \newcite{Levati2017tree} proposed an algorithm to
automatically identify an appropriate threshold from a candidate list for the
reliability of predictions. The automatic selected threshold is to be used in the next iteration of self-training procedure. They scored each candidate threshold by evaluating whether the mean of the out of bag error between the examples with reliability score greater than the considered threshold is
significantly different from the mean of the out of bag error of all the
examples.  


Self-training techniques have also been explored for domain adaptation by some
researchers. For example, \newcite{Ardehaly2016domainadaptation} used self-training process to adapt the label proportion model from the source
domain to the target domain.  \newcite{chattopadhyay2012multisource} generated 
pseudo-labels for the target data. \newcite{daume2008cross} proposed a self
training method in which several models are trained on the same dataset, and
only unlabeled instances that satisfy the cross task knowledge constraints are
used in the self training process.

\newcite{He:2011featureadaptation} derived a set of self-learned and domain-specific features that were
related to the distribution of the target classes for sentiment analysis task. 
Such self-learned features were then used to train another classifier 
by constraining the model’s predictions on unlabeled instances.

Note that although there have been many studies on how to apply self-training to
NLP tasks, all the work design the self-training strategy manually based on the heuristics of the NLP tasks. This makes it difficult to apply these approaches to a different NLP task or a different application scenario. Differently, we propose to design a general self-training approach by learning the self-training
strategy automatically. In this way, our solution can be easily applied to
different application domains.

%{\bf Deep reinforcement learning for NLP} 
There has also been recent work on reinforcement learning for natural language 
processing, such as machine translation \cite{grissom2014don,guo2015generating,gu2016learning,xia2016dual,bahdanau2016actor}, dialog systems \cite{li2016dialogue,su2016continuously}, sentence simplification \cite{zhang2017sentence,narayan2017split}, co-reference resolution \cite{clark2016deep} and latent structure induction \cite{Yogatama2016word2sentence,lei2016rationale}. 
In particular, \newcite{guo2015generating} proposed a deep Q-network model for text generation in sequence-to-sequence models. \newcite{fang2017activelearning} leveraged reinforcement learning for active learning, where a deep Q-network was used to learn the query policy for the active learners.  
%. For example, \newcite{su2016continuously} combined reinforcement learning with
%neural generation on tasks with real users, showing that reinforcement learning
%improves dialogue performance.\newcite{clark2016deep} applied reinforcement
%learning to directly optimize a neural mention-ranking model for co-reference
%evaluation metrics. xxx~\cite{} investigate knowledge transferring from source
%domain to target domain through.... 
%\newcite{Yogatama2016word2sentence} used reinforcement learning to induce implicit syntax structures via auxiliary tasks. \newcite{lei2016rationale} extracted rationales for sentiment prediction and question retrieval tasks. 
However, to the best of our knowledge, there has been no previous attempt to
embed self-training to deep reinforcement learning framework. 
The active learning work of \newcite{fang2017activelearning} is most similar to ours. However, different from active learning which needs to query human experts or oracle to provide gold labels,  
self-training associates instances with automatic prediction label. This makes our work substantially different from that of \newcite{fang2017activelearning}. 





%active learning (\cite{fang2017activelearning})


